On Pre-trained Language Models for Antibody

Antibodies are vital proteins offering robust protection for the human body from pathogens. The development of general protein and antibody-specific pre-trained language models both facilitate antibody prediction tasks. However, there have been limited studies that comprehensively explore the representation capability of distinct pre-trained language models on different antibody tasks. To investigate the problem, we aim to answer several key questions in this paper, such as how pre-trained language models perform in antibody tasks with different specificity and how introducing specific biological mechanisms to the pre-training process can benefit the model. Additionally, we evaluate if the learned antibody pre-trained representations can be applied to real-world antibody problems, like drug discovery and immune process understanding. Previously, no benchmark available largely hindered the study to answer these questions. To aid in our investigation, we provide an AnTibody Understanding Evaluation (ATUE) benchmark. We comprehensively evaluate the performance of protein pre-trained language models by empirical study along with conclusions and new insights. Our ATUE and code are released at https://github.com/dqwang122/EATLM.

==> [arxiv] Antibody/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> [arxiv] Antibody/sections/000abstract.tex <==
% Antibodies are vital proteins that enable robust recognition and removal of harmful pathogens, such as SARS-CoV-2. 
% How we can obtain informative representation of antibody from massive sequence data is crucial for biological understanding and AI-driven drug development. Recent researches view antibody as texts and employ self-supervised language models for representation learning. 
% % When stimulated by the pathogen, immature B cell are mutated into mature antibodies binding this specific pathogen.
% Recently, inspired by the success of protein language models, researchers start to apply those pre-training approaches in learning informative representation for antibodies. However, existing work makes little use of the distinctive evolution process of antibodies that gives them specificity and determines their biological functions.
% However, antibody specific evolution information, which has been long studied in computational biology approaches, were not considered in these approaches. 
% In this work, we improve the antibody representation learning by incorporating the biological evolution process. 


% Antibody representation learning has attracted increasing interest for its potential strength to benefit the fundamental understanding of disease and therapeutic antibody development. Nevertheless, two issues impede the usage of antibody representation learning in real scenarios: existing methods cannot sufficiently extract the biological information of antibody; and the lack of reliable evaluation benchmarks. In this paper, we propose \textbf{E}volution-aware \textbf{A}ntibody \textbf{L}anguage \textbf{M}odel (\method) to incorporate antibody-specific evolution information into pre-training, which can efficiently capture the ancestor relationship between sentences as well as detect mutation during the evolution process. We also provide \textbf{A}n\textbf{T}ibody \textbf{U}nderstanding \textbf{E}valuation (\benchmark) benchmark with six tasks across three major areas of antibody biology. \method achieves excellent performance on these tasks. Further analyses illustrate that the learned evolutionary scope can benefit biological understanding and effective for therapeutic antibody discovery. 


%Antibodies are vital proteins that enable robustly recognition and removal of harmful foreign pathogens, such as SARS-CoV-2. Recently, pre-training language models for antibody representation learning have attracted increasing attention. However, current researches do not make full use of biological information in the antibodies, and the lack of reliable antibody evaluation benchmarks hinders further exploration. In this paper, we propose Evolution-aware Antibody Language Model(EATLM) to incorporate the evolution information into pre-training, which models the ancestor relationship between sentences and capture the mutation during the evolution process. We also provide AnTibody Understanding Evaluation (ATUE) benchmark with six relevant tasks across three different biological domains. EATLM achieve excellent results on these tasks and further analyses illustrate that the learned evolutionary scope can benefit antibody understanding and discovery.


%Recently, pre-training language models for antibody representation learning have attracted increasing attention. However, current researches do not make full use of biological information in the antibodies, and the lack of reliable antibody evaluation benchmarks hinders further exploration. 



% ancestor B cell sequences (germline) into the antibody self-supervised pre-training to learn an evolution representation. Specifically, we concatenate the antibody sequence with its germline and design two auxiliary tasks: contrastive germline classification and somatic mutation prediction. 
% To facilitate the antibody field, we standardize six relevant tasks across three different biological domains and benchmark several recent work on them. Experimental results show that our \textbf{E}volution-aware \textbf{A}ntibody \textbf{L}anguage \textbf{M}odel (\method) outperforms state-of-the-art feature engineering methods, and have better results than existing pre-training models in most cases. The detailed analyses show that our model can better capture the evolution relationship, which helps us decipher the antibody biological function.

Antibodies are vital proteins offering robust protection for the human body from pathogens. The development of general protein and antibody-specific pre-trained language models both facilitate antibody prediction tasks. However, there have been limited studies that comprehensively explore the representation capability of distinct pre-trained language models on different antibody tasks. To investigate the problem, we aim to answer several key questions in this paper, such as how pre-trained language models perform in antibody tasks with different specificity and how introducing specific biological mechanisms to the pre-training process can benefit the model. Additionally, we evaluate if the learned antibody pre-trained representations can be applied to real-world antibody problems, like drug discovery and immune process understanding. Previously, no benchmark available largely hindered the study to answer these questions. To aid in our investigation, we provide an \textbf{A}n\textbf{T}ibody \textbf{U}nderstanding \textbf{E}valuation (\benchmark) benchmark. We comprehensively evaluate the performance of protein pre-trained language models by empirical study along with conclusions and new insights. Our \benchmark and code are released at https://github.com/dqwang122/EATLM.

%Antibody, as a specific type of protein, has attracted increasing interest using pre-trained language models (PLMs) for its potential strength to benefit the fundamental understanding of disease and therapeutic antibody development. However, although several PLMs have been developed specific for antibodies, until now the performance and impact of PLMs on the antibody prediction tasks were rarely empirically explored. We aim to answer the following key questions: (1)Can PLMs sufficiently learn biologically meaningful antibody representation? (2) Do PLMs help antibody tasks? (3) Are antibody specific language model superior to protein PLMs for antibody tasks? (4) If yes, can antibody-specific evolution incorporation benefit prediction? In this paper, we provide an \textbf{A}n\textbf{T}ibody \textbf{U}nderstanding \textbf{E}valuation (\benchmark) benchmark. We comprehensively evaluate antibody and protein PLMs by empirical study along with new insights and conclusions. 






==> [arxiv] Antibody/sections/001introduction.tex <==
Antibodies are a type of protein that is useful for diagnosing and treating a variety of diseases, including SARS-CoV-2~\citep{zhu2022international}. It is crucial to understand the information contained in antibody sequences to develop effective therapeutic antibodies and advance our understanding of the immune system ~\citep{greiff2020mining,lu2018beyond,yermanos2018tracing}. Recent advances in general \textbf{P}re-trained \textbf{P}rotein \textbf{L}anguage \textbf{M}odels~(PPLM) and specific \textbf{P}re-trained \textbf{A}ntibody \textbf{L}anguage \textbf{M}odels~(PALM) offer new possibilities for antibody-related tasks. For example, PPLMs have shown promising results in transferring learned representations to antibody tasks~\citep{kim2021analysis,zaslavsky2022disease} and PALMs have been found to improve model performance in antibody paratope predictions~\citep{leem2022deciphering}.
\begin{wrapfigure}[14]{r}{0.4\linewidth}
    \vspace{-3pt}
    \centering
    \!\!\!\!\!\!\!\includegraphics[width=0.40\textwidth]{figs/intro.pdf}
    \vspace{-5pt}
    \caption{Performance of pre-trained language models on tasks with different antibody specificity.}
    \label{fig:grad}
\end{wrapfigure} 

Despite these successes, few studies have thoroughly examined the capability of different pre-trained language models  (e.g. general PPLMs and specific PALMs) on various antibody tasks, which hinders the development of better architectures for antibody discovery and modification.
To investigate this problem, we compared the performance of the pre-trained protein language model ESM~\citep{rives2021biological}, the pre-trained antibody language model AntiBERT~\citep{leem2021deciphering}, a pre-trained antibody language model EATLM by introducing antibody specific mechanisms, and a model trained from scratch (No Pretrain) on three antibody tasks with varying levels of specificity. The result is illustrated in Figure \ref{fig:grad}.
% For example, in Figure \ref{fig:grad}, we compare the performance of the pre-trained protein language model ESM~\citep{rives2021biological}, the pre-trained antibody language model AntiBERT~\citep{leem2021deciphering}, and the model trained from scratch on three antibody tasks. 
% These three tasks range from low to high in terms of antibody specificity. 
Here, specificity refers to the antibody's unique evolution processes distinct from that of protein to obtain functionality, such as the ability to bind antigen (The definition is discussed in detail in \S \ref{sec:background}).
% A simple experimental result in Figure 1 further highlights the importance of the above problem. We compared the performance of widely used PPLMs and PALMs on three antibody tasks. 


We can see that while ESM performs well in tasks that are less antibody specific, its performance decreases significantly in tasks that are more specific. Additionally, AntiBERT does not demonstrate a clear advantage over the non-pre-trained model in the high-specificity task. These results highlight the limitations of current pre-training language models for antibody-related studies. Using general PPLM representations directly may harm performance, and current pre-training strategies for PALMs may not fit the specific biological functions of antibodies. This emphasizes the need for a comprehensive model design guideline for various antibody tasks. Our main focus is to address the following questions:
% It can be observed that although ESM performs well in task that has low relevance with antibodies, the performance dramatically degrades in tasks of higher relevance. 
% Besides, AntiBERT does not show clear advantages over the non-pretrain model in the high-specificity task. The results point out the weaknesses of current pre-training language models for antibody studies: Direct adaptation of general PPLM representations may damage the performance; Pre-training strategies for PALMs cannot fit the specific antibody biological function well. All of these call for a comprehensive guideline of model designing for different antibody tasks. Mainly, we focus on answering the following questions:
% It can be observed that AntiBERT can generally help antibody prediction, while ESM's performance dramatically varies among different antibody tasks. This result points out that existing studies that directly use representation learned from pre-trained language models for antibodies are dangerous:(1) General PPLM cannot consistently benefit antibody tasks, sometimes is deleterious (Task 3). (2) Even for PALM, the improvement of Task 3 is not significant. 




% \begin{figure}
%     \centering
%     \includegraphics[width=0.7\textwidth]{figs/intro.pdf}
%     \caption{Performance of pre-trained language models on tasks with different specificity. ESM-1 belongs to PPLMs and AntiBERT belongs to PALMs. EATLM is the method with a specific antibody mechanism introduced.}
%     \label{fig:grad}
% \end{figure} 



%Inspired by the recent remarkable success of self-supervised representation learning in proteins, However, the impact of general protein pretrined language m Some researchers aim to develop antibody-specific pretrained language models by viewing the antibody sequences as biological language with a vocabulary of 20 amino acids~\citep{prihoda2022biophi,olsen2022ablang,leem2022deciphering}. Despite of the applications of PPLMs and a range of different PALMs developed, the performance and impact of pretrained language model for antibody is rarely empirically explored. 




%In particular, evolution, described by sequence-sequence relationships between ancestor and progeny antibodies, reflects antibodies' key antigen-binding function ~\citet{honjo1985origin}. Evolution starts from random recombination of V-, D- and J-gene segments to form ancestor sequences, which are germlines ~\citet{tonegawa1983somatic}. Upon exposure to a pathogens, the germlines undergoes frequent mutations, termed somatic hypermutation, to search for progeny sequences with optimal binding specificity ~\citet{nadel1997nucleotide,di2007molecular}. It is known that the complexity of the sequence relationship directly correlates with antibody 's binding specificity to certain antigens ~\citet{conti2019estimation}. Sequence evolution analysis has been employed by many computational biology studies and shows promising results in antibody-related tasks, such as disease diagnosis and therapeutic antibody development ~\citet{yermanos2018tracing, miho2019large}. 

%Fortunately, the recent advent of high-throughput sequencing has led to an exponential increase in unlabeled antibody sequences ~\citet{georgiou2014promise}. The total number of sequences has doubled from 70 million to 1.5 billion in the last five years, providing a gold mine for data-driven unsupervised learning~\citet{kovaltsuk2018observed,olsen2022observed,marks2020repertoire}. 


%Protein sequences can be described as a biological language with a vocabulary of 20 amino acids. Similar to natural languages, structural and functional information are entirely stored in protein sequences with high efficiency. \textbf{P}retrained \textbf{P}rotein \textbf{L}anguage \textbf{M}odels (PPLMs), pretrained on tens of millions to billions of unlabeled protein sequences, have achieved promising progresses in extracting structural and functional information from sequences and become the state-of-the art in predicting general protein applications, including structure and fitness prediction. 

%Despite of the remarkable progress of PPLMs in general protein applications, its performance and impact on specific types of proteins showing unique biological mechanism is rarely empirically explored. Among different types of proteins, antibody is one of the most important subtypes of protein, extensively used as diagnostic and therapeutic tools against diverse diseases in real world, such as SARS-CoV-2. Moreover, antibody 's evolution characteristics is highly specific and significantly different from that of general proteins, providing an good opportunity to study the transfer learning capacity of PPLMs from general problems to specific domain. 

% Notably, although antibody belongs to one out of many protein subtypes, its evolution mechanism is highly specific and significantly different from that of general proteins. The potential hypothesis could be antibody specificity really matters. For tasks requiring low antibody-specific characteristics, PPLM and PALM show comparable performance. For tasks requiring high antibody-specific characteristics, PALM out performs PPLM significantly. 
% Understanding the underlying mechanisms of the results is important to guide further study for antibody representation learning as well as antibody biology?. 
% To investigate the mechanisms, we aim to answer the following key questions. Deciphering these questions is beneficial to both artificial intelligence and biology communities.  

% \textbf{(1) Does the performance of different pre-trained language models highly depend on the antibody specificity underlying downstream tasks?} 
\textit{(I) How well will pre-trained language models perform on antibody tasks with varying specificity?} 
%Despite of the success of PPLMs in general protein predictions, few trials are put into an empirical investigation for PPLMs' effectiveness on antibody downstream tasks, which certainly hindered our understanding of the transfer learning capability of PPLMs on antibody prediction. 
Addressing of the question is mainly hindered by two challenges: the lack of a reliable antibody-specific benchmark for performance evaluation and comprehensive studies of current PPLMs and PALMs.
\textit{(II) Can incorporating biological mechanisms, specifically antibody-specific evolution, into the pre-training process provide additional benefits for antibody representation learning?} This idea has been explored in several computational biology studies, which have demonstrated promising results in antibody-related tasks such as disease diagnosis and therapeutic antibody development~\citep{yermanos2018tracing, miho2019large}.
% Many computational biology studies have shown promising results when incorporating antibody-specific evolution in antibody tasks, such as disease diagnosis and therapeutic antibody development~\citep{yermanos2018tracing, miho2019large}. 
Then, it is interesting to know whether antibody representation learning can benefit from the incorporation of antibody-specific evolution information.
% (shown in red dashed line in figure one). % 
\textit{(III) Are the pre-trained antibody representations useful in practical applications, such as drug discovery and immune process understanding?} Antibodies are critical in drug development, and it is essential to determine whether pre-training representations can be beneficial for biologists to comprehend antibody functions or develop drugs.
% Since antibody is so important that is extensively used for drug development in the real world, it is interesting to know whether pre-trained representation can indeed help biologists to understand antibody functions or discover drugs. 



%Recent studies have shown PLMs self-supervised pre-training on billions of protein sequences can learn the general semantics for proteins and benefit structure and function prediction, which further shed light on the potential usage of PLMs for antibody function prediction.
%Recently, inspired by the the remarkable success of self-supervised learning from natural language processing, many researchers view the antibody sequences as a biological language with a vocabulary of 20 amino acids~\citep{prihoda2022biophi,olsen2022ablang,leem2022deciphering} and modeled using PLMs. 
%Interesting results for antibody analysis have been achieved. AbLang~\citet{olsen2022ablang} introduced an antibody language model that can restore missing residues of antibody sequences. AntiBERTy~\citet{ruffolo2021deciphering} use the redundancy, which indicates the frequency of the occurrence of antibody sequences in an immune response, as a weak supervised signal for binding capability. 


%\textbf{Q(1): Can existing PLMs sufficiently learn the biologically meaningful representations of antibody?} Existing antibody PLM mainly adapt masked language modeling to antibody sequences, which effectiveness are barely known.

%\textbf{Q(2): Do PLMs help antibody tasks?} Despite of a series of antibody PLMs developed, few trials are put into empirical investigation for PLMs' effectiveness on antibody downstream tasks~\citep{olsen2022ablang,ruffolo2021deciphering}. Two key challenges faces the study: a reliable benchmark for comprehensive performance evaluation is lacking; the computational cost training these large models from scratch is out of reach in most academic research groups. 

To investigate these questions, we first propose antibody study benchmark \textbf{A}n\textbf{T}ibody \textbf{U}nderstanding \textbf{E}valuation (\textbf{ATUE}). This is the first antibody benchmark with four real-world supervised tasks related to therapeutic antibody engineering, B cell analysis, and antibody discovery. These tasks cover a range of specificity levels to evaluate models on different aspects of antibody biological functions.
% To evaluate models on different aspects of antibody biological functions, these tasks are designed to have specificity ranging from low to high. 
Based on \benchmark, we conduct empirical studies to investigate the representation ability of distinct pre-trained language models. To explore the impact of incorporating specific biological mechanisms in antibody pre-training, two objectives are introduced to tailor masked language modeling for evolution:
% These objectives include \textit{Ancestor germline prediction} and \textit{Mutation position prediction}, which are used to investigate the representation ability of an antibody evolution-tailored language model.
% We also explore the influence of involving specific biological mechanisms in antibody pre-training 
% proposing a \textbf{E}volution-aware \textbf{A}ntibody \textbf{L}anguage \textbf{M}odel (\textbf{EATLM}). We 
% by introducing two simple objectives to tailor masked language modeling for evolution: 
(1) \textbf{Ancestor germline prediction} guides the model to discriminate the evolutionary relationship between antibody and ancestral sequences. (2) \textbf{Mutation position prediction} mimics hypermutation during the evolution. These methods are used to investigate the representation ability of antibody evolution-tailored language model.
% , predicts mutation positions and residues. It is the first attempt to incorporate antibody evolution information into the pre-training framework. %We introduce two tasks to tailor masked language modeling for evolution: (1) Ancestor germline prediction (\CGC) guides the model to discriminate the evolutionary relationship between antibody and germline sequences. (2) Mutation position prediction (\MPP), mimicking somatic hypermutation during the evolution, predicts mutation positions and residues. 
% For Q3, we compare the performance of various pretrained models on SARS-CoV-2 antibody discovery. 
Finally, we take a close look at the SARS-CoV-2 antibody discovery to investigate the pre-trained representation under a real-world scenario.

% Our empirical study contributes to artificial intelligence and antibody biology fields by providing the following conclusions and insights:
We have three main contributions in this study:
\begin{itemize*}
    \item We created the first comprehensive antibody benchmark called \benchmark to help with antibody application studies, which includes four real-world supervised tasks ranging from low to high specificity. We also introduce two new objectives for antibody pretraining that incorporate antibody-specific evolutionary information.
    % \item For facilitating antibody application studies, we develop the first comprehensive antibody benchmark to benefit the community. 
    % This is the first attempt to show how antibody-specific evolutionary information can be incorporated into the pre-training language model.
    % We also introduce two new objectives for incorporating antibody-specific evolutionary information into antibody pretraining.
    % \item For providing guidelines for a better antibody representation, we have the following key observations: \textbf{(i)} \textit{PPLMs perform well on antibody tasks that have a high relationship with structure.} However, they perform worst in tasks with high antibody specificity, indicating representation benefiting protein structure prediction is harmful to antibody-specific tasks. \textbf{(ii)} \textit{In most cases, PALMs perform as well as or even better than PPLMs with less pre-training data.} \textbf{(iii)} \textit{PALMs can be improved by incorporating the evolution process.} However, the evolution information from MSAs does not always benefit the antibody tasks. 
    \item We made key observations for providing guidelines for better antibody representation. Firstly, PPLMs perform well on antibody tasks that have a high relationship with structure, but they perform poorly on tasks with high antibody specificity. Secondly, in most cases, PALMs perform as well as or even better than PPLMs with less pre-training data. Thirdly, PALMs can be improved by incorporating the evolution process, but the evolution information from MSAs does not always benefit antibody tasks.
    % \textbf{(iv)} The introduction of two antibody biological mechanisms facilitates PALMs with more antibody-specific features and improves model performance in the task with high antibody specificity. 
    % The performance of PPLMs depends on the antibody specificity relatedness of downstream tasks. PALMs significantly outperform PPLMs for antibody tasks with high antibody evolution relatedness, suggesting general protein pre-trained models are not sufficient in antibody-specific representation learning. \textbf{(2)} Antibody-specific evolution incorporated pre-trained language model can significantly improve the effectiveness of representation learning on downstream tasks. Future study to have more in-depth research in this direction would be interesting. 
    % \textbf{(3)} Improvement on antibody representation can further facilitates real-world scientific discovery of clinically useful antibodies against SARS-CoV-2. %Using the language model, we identified 38 potential SARS-CoV-2 binders which sequences are highly identical to therapeutic antibodies known to bind the virus.
    % \item For accelerating real-world antibody discovery, we identified 11 potential SARS-CoV-2 binders whose sequences are highly identical to existing therapeutic antibodies binding with the virus.
    \item We identified 11 potential SARS-CoV-2 binders that have highly identical sequences to existing therapeutic antibodies that bind to the virus, which could accelerate real-world antibody discovery.
\end{itemize*}
% Antibodies are vital proteins produced by the immune system offering robust protection for human body from harmful pathogens. Antibodies have been extensively used as diagnostic and therapeutic tools against diverse diseases, such as SARS-CoV-2~\citet{zhu2022international}. To perform its protective function, antibody sequence undergoes evolution selection to search for optimal patterns that can specifically recognize pathogens~\citet{honjo1985origin}. Deciphering the information stored in antibody sequences can benefit our understanding of disease and accelerate therapeutic antibody development ~\citet{greiff2020mining,lu2018beyond,yermanos2018tracing}. 


% However, two key challenges impede the usage of representation learning for antibody analysis. First, despite several studies of antibody representation learning, a reliable benchmark for comprehensive performance evaluation is very much lacking, which certainly hinders future research in antibodies ~\citep{olsen2022ablang,ruffolo2021deciphering}. Second, the existing methods view antibody sequences as texts and simply adopt masked language modeling for representation learning ~\citep{olsen2022ablang,ruffolo2021deciphering}. We argue this formulation of pre-training cannot sufficiently and efficiently extract antibody biological information, which is crucial for many antibody functions. 

% In particular, evolution, described by sequence-sequence relationships between ancestor and progeny antibodies, reflects antibodies' key antigen-binding function ~\citet{honjo1985origin}. Evolution starts from random recombination of V-, D- and J-gene segments to form ancestor sequences, which are germlines ~\citet{tonegawa1983somatic}. Upon exposure to a pathogens, the germlines undergoes frequent mutations, termed somatic hypermutation, to search for progeny sequences with optimal binding specificity ~\citet{nadel1997nucleotide,di2007molecular}. It is known that the complexity of the sequence relationship directly correlates with antibody 's binding specificity to certain antigens ~\citet{conti2019estimation}. Sequence evolution analysis has been employed by many computational biology studies and shows promising results in antibody-related tasks, such as disease diagnosis and therapeutic antibody development ~\citet{yermanos2018tracing, miho2019large}. 

% Fortunately, the recent advent of high-throughput sequencing has led to an exponential increase in unlabeled antibody sequences ~\citet{georgiou2014promise}. The total number of sequences has doubled from 70 million to 1.5 billion in the last five years, providing a gold mine for data-driven unsupervised learning~\citet{kovaltsuk2018observed,olsen2022observed,marks2020repertoire}. Large-scale pre-training language models have shown powerful strength in extracting information from massive unlabeled sequences~\citet{sarzynska2021detecting,devlin2018bert,radford2019language}, offering a unique opportunity to learn the general biological semantics for antibody sequences. To explore this idea, two studies, AbLang~\citep{olsen2022ablang} and AntiBERTy~\citep{ruffolo2021deciphering}, recently developed antibody self-supervised pre-training antibody language models, and achieved promising results in understanding the biological characteristics.

% Antibodies are composed of two identical heavy chains and two identical light chains, forming a large Y-shaped structure, where the two tips are responsible for pathogens binding (Figure \ref{fig:evolution}).  During evolution, the initial diversity is encoded into the ancestor sequence through randomly recombination of V-, D- and J-gene segments. Upon exposure to a pathogen, the sequence undergoes frequent sequence mutations to search for progeny sequences with optimal binding specificity. Decoding the sequence evolution patterns using machine learning methods has shown promising results that benefit many antibody-related tasks, such as disease diagnosis (ref) and therapeutic antibody development (ref). 
% Inspired by the success of masked language modeling in natural language processing, many researchers view the antibody sequences as a biological language with a vocabulary of 20 amino acids~\citep{prihoda2022biophi,olsen2022ablang}.
% Based on this, ~\citet{ruffolo2021deciphering} use the redundancy, which indicates the frequency of the occurrence of antibody sequences in an immune response, as a weak supervised signal for binding capability. 
%However, the masked language modeling just capture the distribution of amino acid, and the small vocabulary and frequent mutation of antibody make the distribution more even than natural languages. Thus, it can provide less information than language contexts and does not provide biological insights.



%In particular, mask language models cannot learn the critical evolution features of antibody, which defines the sequence-sequence relationships between ancestor and progeny antibodies. The complexity of the evolutionary relationship reflects important antibody functions correlating with the breadth of antigen-binding (Figure 1) (ref). Evolution architecture analysis, e.g., phylogenetic inference, by measuring sequence similarity between the observed antibodies and their common ancestors, has been employed in computational biology tools to discriminate antibody repertoires between health and disease (ref). Hence, it is necessary to introduce the 
% evolution information into the model for better antibody representation.


% However, little work takes the evolutionary process into consideration when learning the representation38of antibody sequences. There are two key challenges. The first is to formulate and model the complex39evolutionary process into the pre-training framework. It includes the relationship between ancestor sequences and descendant antibodies with binding specificity. Besides, the mutation positions and tokens have a great influence on the biological functions of antibody sequences. Second, the lack of42reliable benchmarks for the comprehensive performance evaluation has hindered development in this43area. Different from protein, which has several universally accepted supervised tasks and standard44benchmarks (Rao et al., 2019), existing pre-training methods only conduct qualitative analysis. Most45of them just conduct some visualization or recover masked tokens, and do not compare with other46work. It is highly necessary to design a benchmark to incentivize and guide future research in47antibodies.


% impede the usage of representation learning in antibody sequence pattern analysis. 
% First, existing antibody representation methods view antibody sequences as texts and simply explore mask language models for representation learning (ref). This formulation of pre-training is insufficient in capturing the information embedded in the antibody sequence, especially the evolution relationships. 
% The second challenge is the lack of reliable downstream benchmarks, hindering comprehensive performance evaluation for transfer learning. Existing pre-training methods were evaluated only on the tasks of preliminary analysis, such as visualization, missing sequence restoration, and potential antigen-binding site identification (ref). It is highly necessary to design a benchmark to incentivize and guide future research in antibodies.

%To address these challenges, this paper proposes \textbf{E}volution \textbf{A}ntibody \textbf{L}anguage \textbf{M}odel (\method), which is the first to incorporate antibody evolution information into the pre-training framework. We introduce two tasks to tailor masked language modeling for evolution: (1) Ancestor germline prediction (\CGC) guides the model to discriminate the evolutionary relationship between antibody and germline sequences. (2) Mutation position prediction (\MPP), mimicking somatic hypermutation during the evolution, predicts mutation positions and residues. 
%Besides, We build the first antibody study benchmark \textbf{A}n\textbf{T}ibody \textbf{U}nderstanding \textbf{E}valuation (\benchmark) to quantitatively evaluate the performance of the antibody representation. Six biologically relevant supervised tasks are included, requiring different levels of sequence understanding. These tasks comprehensively highlights three major aspects of antibody applications: B cell analysis, disease diagnostics and therapeutic antibody development. Improvement on these tasks can further facilitates the scientific discovery of clinically useful antibodies against viruses. Remarkably, we found 2 true and 35 potential B cell antibodies targeting diverse epitopes of SARS-CoV-2.

%For quantitative comparison, we build a B-cell antibody study benchmark considering both biological impacts and task diversity. This is the first evaluation suite for B-cell antibodies comprising five datasets, which require different levels of sequence understanding and comprehensively cover two important aspects of antibody application: disease diagnosis and B-cell monoclonal antibody development.

% antibody ancestor sequences into the unsupervised representation learning, which is the first general framework exploring the evolutionary scope shown by the representation. We analyze our antibody language model through the lens of attention and present a set of interpretability methods that capture the unique evolution and function of antibodies. To evaluate the pretraining method, we introduce the B-cell antibody study benchmark by collating the current research thread in this area. This is the first evaluation suite for B-cell antibodies comprising five datasets, which require different levels of sequence learning and comprehensively cover two important aspects of antibody application: 1) disease diagnosis; 2) B-cell monoclonal antibody development. One-shot, Few-shot? 

%Our contribution is three-fold: (1) We propose \method, which is the first evolution embedded antibody pre-training approach. The training objectives \CGC and \MPP model the biological process of the evolution from sequence and residue level. (2) We construct and release \benchmark, the first antibody benchmark, facilitating antibody application study in three aspects: B cell analysis, disease diagnostics, and therapeutic antibody engineering. \method showed excellent improvements on these tasks. \method is effective for therapeutic antibody discovery, by finding potential antibodies for SARS-CoV-2 treatment. (3) We provide an interpretable analysis and explore the evolutionary scope shown by the representation, which can benefit antibody evolution understanding, such as tracing antibody maturation. 



%Large-scale language models (PLM) have improved the performance in protein prediction tasks, such as structure prediction and protein engineering. Encouraged by the promising results, increasing interest have been attracted to apply pre-training language model on antibody, a specific type of protein critical for disease diagnosis and drug development.






==> [arxiv] Antibody/sections/002related.tex <==
Our work focuses on researching the effectiveness of protein and pre-trained antibody language models for antibody-specific tasks. Below we review the representative existing methods. We list the details in Table \ref{tab:PLMs}. 

\textbf{Pretrained Protein Language Models (PPLMs)} There is an increasing interest in exploring large-scale language models using protein sequences~\citep{rao2019evaluating,madani2020progen,meier2021language,chen2022structure}. These models have been shown to achieve state-of-art capacity in predicting protein structure and function. ProtTrans~\citep{elnaggar2021prottrans} and ESM-1b~\citep{rives2021biological} take individual protein sequences as input and adopt Transformer language models for pre-training, demonstrating that self-supervision is a promising paradigm for protein secondary structure, contact, homology predictions, and function prediction. To extract evolutionary information from protein sequences, \citet{rao2021msa} proposed the MSA-transformer/MSA-1b model utilizing multiple sequence alignment (MSA) instead of a single query sequence as input. This model is superior to ESM-1b for structure prediction, demonstrating evolution information can benefit protein representation learning. Despite the progress in the field, few studies reported their results on antibody tasks. 

\textbf{Pretrained Antibody Language Models (PALMs)} Encouraged by the success of PLMs in protein representation learning, series work seeks to learn antibody representations based on sequences of antibodies. 
% ~\citep{leem2021deciphering,olsen2022ablang,prihoda2022biophi,li2022antibody}. 
AntiBERTy~\citep{ruffolo2021deciphering} proposed the first antibody-specific language model, exploring a Transformer trained on 558M natural antibody sequences in the OAS database. 
% The case study in the work showed the representation obtained from the PLM is useful for antibody sequence clustering into trajectories resembling affinity maturation. 
\citet{olsen2022ablang} train two language models for antibodies: A heavy chain version Ablang-H and a light chain version Ablang-L. The study reported transfer learning results on restoring missing residues of antibody sequences, which is a task similar to pre-training objectives. 
AntiBERTa~\citep{leem2021deciphering} train the antibody language model on OAS and finetuning AntiBERTa for paratope position prediction, achieving state-of-the-art performance.
% , the experimental results lack standard deviations, making it unclear how significant the results obtained are. 
Recently, \citet{li2022antibody}  proposed an antibody-specific language model and explored its performance in SARS-CoV-2 antigen binding, showing context-dependent representations of antibody sequences benefit binding prediction.

\input{tabs/PLMs}



%Second, the complexity of pre-training on antibodies are insufficient to antibody biological information. Existing studies view antibody sequences as texts and simply adopt masked language modeling for representation learning. 
%To interpret the language model, Vig et al, proposed a set of methods for protein Transformer attention analysis and found attention from different layers can capture the unique functional and structural characteristics of proteins~\citet{vig2020bertology}. \citet{elnaggar2021prottrans} explored the limits of up-scaling language models trained on proteins. \citet{zhang2022ontoprotein} construct large-scale knowledge graphs consisting of gene ontology biologic knowledge and incorporate it into protein pretraining. 


% Phylogenic tree analysis


==> [arxiv] Antibody/sections/003task.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=0.9\linewidth]{figs/task.pdf}
%     \caption{Tasks on antibody. (A).  (B)  (C)}
%     \label{fig:task}
% \end{figure}

%This section gives an overview about antibody and relevant tasks. First, we give a detail introduction of antibody and its evolution mechanism, as the biological guidelines for our method. Then, we propose the AnTibody Understanding Evaluation (ALUE) benchmark, which is the rst standardized evaluation suit for antibody.

% \subsection{Antibody with Evolution Information}


In this section, we first give a brief introduction to the antibody and its specific evolution. Then we propose the first antibody-specific benchmark (\benchmark) composed of four tasks with different specificities. Finally, we implement several PPLMs and PALMs baselines and design an evolution-aware PALM to incorporate the biological mechanism into the pre-training process.

\subsection{Background}
% Antibody Definition + Evolution relationship
\label{sec:background}
\textbf{Antibody} Antibodies are vital proteins generated by the immune system to remove harmful foreign pathogens in the human body. they can specifically bind to antigens on the pathogen and recognize it. Antibodies are composed of two identical heavy chains and two identical light chains and form a large Y-shaped structure. Two tips on it contain highly variable loops, called Complementarity Determining Regions (CDR), which function for antigen binding. 

\textbf{Antibody Specific Evolution} Notably, the antibody evolution process is significantly different from that of proteins, providing a good opportunity for us to investigate the impact of general PPLMs on specific subdomains. To perform its protective function, the antibody sequence undergoes evolution selection to search for optimal patterns that can specifically recognize pathogens~\citep{honjo1985origin}. Deciphering the information stored in antibody sequences may benefit our understanding of disease and accelerate therapeutic antibody development~\citep{greiff2020mining,lu2018beyond,yermanos2018tracing}. During evolution, the random recombination of V/D/J-gene segments provides the initial diversity for the ancestor sequence (germline). Upon exposure to a pathogen, this sequence undergoes frequent sequence mutations to search for progeny antibody sequences with optimal binding specificity. In other words, gene recombination provides millions of germlines in the human body, and the germlines further mutate into a huge number of progeny antibodies. Thus, the ancestor relationship between an antibody and its corresponding germline as well as the mutation it undergoes together determine the unique biological functions. In brief, the evolutionary relationships between antibodies arise to gain new functions such as antigen binding. It is significantly different from that of proteins, which are to maintain certain functions across different organisms. We further illustrate this process in Figure \ref{fig:evolution} in \S \ref{sec:evolution}.
%Therefore, it is necessary to develop an antibody evolution aware PLM to better capture the biological characteristics of antibody sequences.


% Antibodies are composed of two identical heavy chains and two identical light chains, forming a large Y-shaped structure, where the two tips are responsible for pathogens binding (Figure \ref{fig:evolution}).  During evolution, the initial diversity is encoded into the ancestor sequence through randomly recombination of V-, D- and J-gene segments. Upon exposure to a pathogen, the sequence undergoes frequent sequence mutations to search for progeny sequences with optimal binding specificity. Decoding the sequence evolution patterns using machine learning methods has shown promising results that benefit many antibody-related tasks, such as disease diagnosis (ref) and therapeutic antibody development (ref). 
% Inspired by the success of masked language modeling in natural language processing, many researchers view the antibody sequences as a biological language with a vocabulary of 20 amino acids~\citep{prihoda2022biophi,olsen2022ablang}.


%\textbf{Pairing Antibody with Germline} 
%To obtain the evolutionary information of antibody sequences, we utilize Observed Antibody Space (OAS), a database containing more than 1.5 billion natural antibody sequences~\citep{kovaltsuk2018observed,olsen2022observed}. 
%The antibody sequences in the database have been precisely annotated with of evolutionary and structural information, including the paired germline and CDR3 for each antibodies. 

%To pair the antibody sequences with their ancestor germline, we make use of the diverse natural antibody sequence database Observed Antibody Space (OAS)~\citep{kovaltsuk2018observed,olsen2022observed}. It contains more than 1.5 billion annotated repertoire data, including its germline and CDR information. Thus, it is suitable for our evolution-aware pre-training. We downloaded the August 2021 version from its website and remove duplicate sequences. Then, we cluster sequences based on the CDR3 fragment and filter each cluster by 70\% identity over the whole sequence using Linclust~\citep{steinegger2018clustering}. The remaining sequences are divided into 20,245,249 for training and 45,249 for validation. Each sequence have its corresponding ancestor germline sequence.

\textbf{Unsupervised Antibody Corpus}
To obtain the evolutionary information of antibody sequences, we utilize Observed Antibody Space (OAS), a database containing more than 1.5 billion natural antibody sequences~\citep{kovaltsuk2018observed,olsen2022observed} The antibody sequences in the database have been precisely annotated with evolutionary and structural information, including the paired germline and CDR3 for each antibody. To pair the antibody with its germline used in the pretraining task, we used the annotated sequences provided in the OAS database. Further information on data processing can be found in \S \ref{sec:data_pro}. 

\subsection{\textbf{A}n\textbf{T}ibody \textbf{U}nderstanding \textbf{E}valuation (ATUE)} 
%\label{sec:benchmark}
We provide four biologically relevant downstream prediction tasks to serve as antibody benchmarks, covering four major application aspects for antibodies in the real world: therapeutic antibody engineering, disease diagnostics, antibody discovery, and B cell maturation analysis. The antibody specificity of these tasks ranges from low to high, offering scaled tasks with subdomain specificity for pre-trained language model evaluation. Detailed information is listed in Figure \ref{fig:benchmark}. All data are publicly open and used under the right license. For each task, we focus on the following aspects and leave the details in Appendix (\S \ref{sec:a_benchmark} and \S \ref{sec:task_specificity}):

\begin{xQuote}
\textbf{[Definition]} The formal definition of the task and the understanding ability required. \\
\textbf{[Impact]} The importance of the task in the biological area.\\
\textbf{[Dataset]} The data source and size. \\
\textbf{[Specificity]} Antibody’s specific evolution characteristics are different from general proteins. 
\end{xQuote}

\begin{figure}
     \centering
%     \begin{subfigure}{0.49\textwidth}
%         \includegraphics[width=\textwidth]{figs/evolution.pdf}
%         \caption{t75.}
%         \label{fig:evolution}
%     \end{subfigure}
%     \hfill
     % \begin{subfigure}{0.98\textwidth}
         \includegraphics[width=\textwidth]{figs/task.pdf}
         \caption{Antibody prediction tasks. The specificity of tasks ranges from low to high.}
         \label{fig:benchmark}
     % \end{subfigure}
 \end{figure}
 
%\input{tabs/task}
% \input{tabs/tasks}

We use several classification metrics to evaluate the performance. Accuracy (\textbf{ACC}) calculates the ratio of correct predictions. Matthews Correlation Coefficient (\textbf{MCC}) is the coefficient between true and predicted values. \textbf{F1} is the average weighted score of precision and recall. \textbf{AUC} is the area under the ROC curve, which shows the performance at all classification thresholds.

\textbf{Antigen Binding Prediction} is a binary sequence classification task to determine whether the CDR region of the antibody can bind to the specific antigen.
\begin{xQuote}
    \textbf{[Impact]} A better understanding of the binding affinity between antibodies and antigens can accelerate the affinity optimization of therapeutic antibodies. \\
    \textbf{[Dataset]} We collect the antigen binding data from ~\citet{mason2021optimization} and follow the training/validation/test split of 15,128/3,242/3,242. \\
    % The paratope data is collected from ~\citet{liberis2018parapred} with 1,662 CDR segments on 277 antibodies. \\
    \textbf{[Specificity]} Low. All the antibodies sequence in the dataset are derived from a single germline sequence indicating the task is not antibody-specific evolution-related. 
\end{xQuote}
    
% \begin{itemize*}
%     \item \textbf{[Impact]} The better understanding of the binding affinity between antibody and antigen can accelerate the affinity optimization of therapeutic antibodies during pharmaceutical drug development. 
%     \item \textbf{[Dataset]} We collect the antigen binding data from ~\citep{mason2021optimization} and follow the training/validation/test split of 15,128/3,242/3,242. The paratope data is collected from ~\citep{liberis2018parapred} with 1,662 CDR segments on 277 antibodies. 
%     \item \textbf{[Specificity]} Low. All the antibodies sequence in the dataset are derived from a single germline sequences indicating the task is not antibody specific evolution related. 
% \end{itemize*}

\textbf{Paratope Prediction} It is to identify binding positions on the antibody sequence, which is a sequence labeling task to predict a 0/1 label for each residue of CDR fragments. 
\begin{xQuote}
    \textbf{[Impact]} The exploration of paratope (binding positions between antibody and antigen) can help to understand the binding mechanisms of therapeutic antibodies. \\
    \textbf{[Dataset]} The paratope data is collected from ~\citet{liberis2018parapred} with 1,662 CDR segments on 277 antibodies. \\
    \textbf{[Specificity]} This task is medium specificity related because only partial antibodies from the database are derived from evolution. 
\end{xQuote}
    
% \begin{itemize*}
%     \item \textbf{[Impact]} The better understanding of the paratope (binding positions between antibody and antigen) can help to understand the binding mechanisms of therapeutic antibodies. 
%     \item \textbf{[Dataset]} We collect the antigen binding data from ~\citep{mason2021optimization} and follow the training/validation/test split of 15,128/3,242/3,242. The paratope data is collected from ~\citep{liberis2018parapred} with 1,662 CDR segments on 277 antibodies. 
%     \item \textbf{[Specificity]} This task is medium specificity related because only partial antibodies from the database are derived from evolution. 
% \end{itemize*}

%\subsubsection{Disease Diagnosis} 
%The disease classification is an individual-level task to map a profile with multiple antibody sequences to a 0/1 label, where 1 indicates that the individual has the disease. This task aims to determine which disease the patient has, requiring the model to capture disease-specific features with extreme imbalance labels full of noise.
%\begin{itemize*}
%    \item \textbf{[Impact]} It helps diagnose infectious and immune related disease without expensive wet laboratory testing. Previous biological studies mainly use this multi-classification task for disease diagnosis ~\citet{zaslavsky2022disease,wang2022large}, highlighting the discriminatory power among different diseases are important for disease diagnosis.
%    \item \textbf{[Dataset]} We filter the disease data from OAS and follow the processing pipeline of ~\citep{kim2021analysis} to handle it. We merge profiles of three virus infection diseases (SARS, HIV, Ebora), three immune-related diseases (allergy, SLE, and MS), and healthy profile for disease classification. For each profile, we use select top100 sequences in redundancy and annotate them with the label of profile to avoid the noise. 
%    \item \textbf{[Antibody specificity]} Disease diagnosis task is antibody specific evolution-related since it is reported antibody derived different disease have specific preferance for different ancestor germlines~\citep{bashford2019analysis}. 
%\end{itemize*}

% \begin{xQuote}
%     \textbf{[Impact]} It helps diagnose infectious and immune related disease without expensive wet laboratory testing. Previous biological studies mainly use this multi-classification task for disease diagnosis ~\citet{zaslavsky2022disease,wang2022large}, highlighting the discriminatory power among different diseases are important for disease diagnosis. \\
%     \textbf{[Dataset]} We filter the disease data from OAS and follow the processing pipeline of ~\citep{kim2021analysis} to handle it. We merge profiles of three virus infection diseases (SARS, HIV, Ebora), three immune-related diseases (allergy, SLE, and MS), and healthy profile for disease classification. For each profile, we use select top100 sequences in redundancy and annotate them with the label of profile to avoid the noise. \\
%     \textbf{[Antibody specificity]} Disease diagnosis task is antibody specific evolution-related since it is reported antibody derived different disease have specific preferance for different ancestor germlines~\citep{bashford2019analysis}. 
% \end{xQuote}
    

% Each human is estimated to maintain ~108-1010 distinct antibody sequences, constructing an informative encyclopedia recording the past and present health and disease. Interpreting the pattern of the sequences has already proved useful in disease diagnosis and allows us to assess many infectious diseases without expensive laboratory testing. 





% \textbf{Antigen Binder Prediction} Antigen binding prediction (Therapeutic antibody engineering)
% \textbf{[Definition]}  Antigen binding is a two-class sequence classification test. The data are collected from this paper (ref).
% \textbf{[Impact]} Therapeutic antibodies have become an important tool in treating numerous diseases, such as COVID-19. Accurate antigen-binding prediction approaches could allow significantly more efficient antibody discovery with higher affinity. Machine learning methods have already achieved some success in antibody binding capacity optimization (ref).
% \textbf{[Generalization]}
% \textbf{[Metric]}


% \textbf{Paratope Prediction} Antigen binding site prediction (Therapeutic antibody engineering)
% \textbf{[Definition]}  Antigen binding is a two-class sequence classification test. The data are collected from this paper (ref).
% \textbf{[Impact]} Paratope is the antibody residues involved in antigen binding. The ability to accurately map the paratope can provide a detailed knowledge about binding mechanism and accelerate antibody discovery. 1D sequence-based deep learning method have been employed for paratope prediction. 
% \textbf{[Generalization]}
% \textbf{[Metric]}




\textbf{B Cell Maturation Analysis} 
It is a 6-category classification task to distinguish the maturation stage of B cell antibody sequences. Each sequence belongs to one of \{\textit{immature, transitional, mature, plasmacytes, memory IgD+, memory IgD-}\}. It requires the model to learn a representation sensitive to different maturation states.
\begin{xQuote}
    \textbf{[Impact]} It benefits the understanding of the mechanism during immune evolution, which is a critical biological process in the immune system affecting the function and antigen specificity of antibodies~\citep{ghraichy2021different,meffre2000antibody}. \\
    \textbf{[Dataset]} We collect 88,094 sequences from ~\citet{mroczek2014differences} with 6 maturation stages. \\
    \textbf{[Specificity]} High. Antibody evolution is highly coupled with B cell maturation~\citep{meffre2000antibody}.
\end{xQuote}
% \begin{itemize*}
%     \item \textbf{[Impact]} It helps a better understanding of the mechanism of immune evolution, which is a critical biological process in the immune system affecting the function and antigen specificity of antibodies~\citet{ghraichy2021different,meffre2000antibody}.
%     \item \textbf{[Dataset]} We collect 88,094 sequences from ~\citet{mroczek2014differences}.
%     \item \textbf{[Specificity]} It is a high specificity task because antibody evolution processes is highly coupled with B cell maturation. 
% \end{itemize*}


\textbf{Antibody Discovery} 
The task is a binary sequence classification task to distinguish which antibody is directly responsible for SARS-CoV-2 binding. The task is highly challenging from two aspects: (1) Less than 1\% of antibodies from SARS-CoV-2 patients are directly responsible for virus binding. (2) It is hard to get a reliable sequence-level classifier using unreliable and noisy individual-level labels.

\begin{xQuote}
    \textbf{[Impact]} Antibody discovery from B cell repertoire has been widely recognized as a important approach to accelerate antibody discovery for diverse antigens~\citep{weiner2015building,pedrioli2021single}, and achieved great success for SARS-CoV-2 antibody discovery~\citep{kovaltsuk2018observed,cao2020potent,shiakolas2022efficient}.\\ %This task aims to identify SARS-CoV-2 direct binding antibodies, providing potential antibody candidates fighting against the ongoing SARS-CoV-2 pandemic. 
    \textbf{[Dataset]} We collected antibody sequences from 133 SARS-CoV-2 patients and 87 health persons from OAS and followed the processing pipeline of ~\citet{kim2021analysis}. Inspired ~\citet{zaslavsky2022disease}, we match the high-ranked sequences with the sequences in the CoV-AbDab~\citep{raybould2021cov} database, which have been proved to bind SARS-CoV-2 using wet-lab experiments. \\
    \textbf{[Specificity]} High. It is widely reported antibodies derived from the same disease such as SARS-CoV-2 share strong convergent germline signals ~\citep{galson2020deep}. 
\end{xQuote}


% \begin{itemize*}
%     \item \textbf{[Impact]} Antibody discovery from B cell repertoire has been widely recognized as a important approach to accelarate antibody discovery for diverse antigens~\citep{weiner2015building,pedrioli2021single}, and achieved great success for SARS-CoV-2 antibody discovery~\citep{kovaltsuk2018observed,cao2020potent,shiakolas2022efficient}. %This tasks aims to identify SARS-CoV-2 direct binding antibodies, providing potential antibody candidates fighting against ongoing SARS-CoV-2 pandamic. 
%     \item \textbf{[Dataset]} We collected antibody sequences from 133 SARS-CoV-2 patient and 87 health persons from OAS and followed the processing pipeline of Kim et al.~\citep{kim2021analysis}. Inspired by the methods in this study \citep{zaslavsky2022disease}, we match the high-ranked sequences with the sequences in the CoV-AbDab~\citep{raybould2021cov} database, which have been proved to bind SARS-CoV-2 using wet-lab experiments.
%     \item \textbf{[Specificity]} This task is high antibody evolution-related since it is reported antibody derived the same disease such as SARS-CoV-2 reveal strong convergent germline signals ~\citep{galson2020deep}. 
% \end{itemize*}










% B-cell maturation prediction has been employed in multiple studies for  (ref) (Figure 2A).
%It is widely reported that changes in antibody sequence patterns correlate with B-cell maturation (ref). Therefore, we use this task to evaluate the representation learning capacity of the language model. 

==> [arxiv] Antibody/sections/004method.tex <==
% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]{figs/22.pdf}
%     \caption{model}
%     \label{fig:model}
% \end{figure}

% Detailed descriptions of this biological mechanism and the evolutionary process can be found in Appendix.
Based on the antibody benchmark \benchmark, we evaluate the performance of current pertaining language models in different specificity tasks. Furthermore, to investigate the benefit of introducing the biological mechanism, we incorporate evolution information as the extra pretraining objectives for PALMs and propose \method. The detailed description of the objective and the implementation can be found in \S \ref{sec:training}


\textbf{Current Pre-trained language models}
Existing antibody and protein language models are summarized in Table \ref{tab:PLMs}. 
% We choose two representative PALMs pre-trained on large-scale antibody sequences, \textbf{Ablang}~\citep{olsen2022ablang}, \textbf{AntiBERTa}~\citep{leem2022deciphering} in this study. 
Since the code and pre-training data of AntiBERTa are not released, we train a BERT model named \textbf{AntiBERT} on the full OAS database following the same setting as the original study. 
% We evaluate two representative PPLMs: ESM\footnote{To make a fair comparison, we use the released base version \textbf{ESM-1}, which has 86M parameters.} and MSA-1b/MSA-Transformer. \textbf{MSA-1b}~\citep{rao2021msa} is a Transformer-based language model taking protein-specific evolutionary sequences (Multiple Sequence Alignment, MSA) as the input to get context embeddings. 
% MSA-Transformer outperforms ESM-1b for protein structure prediction. 
\textbf{MSA-1b}~\citep{rao2021msa} takes protein-specific evolutionary sequences (Multiple Sequence Alignment, MSA) as the input. Because it is hard to align sequences between antibodies due to the diversity of CDR3, we take the germline and create pseudo-MSAs with depth 2. 
We add a linear layer on top of the language models and finetune the whole model on the downstream tasks.



%We implement \method as described in Section \ref{setup}. We also conduct ablation studies that remove \CGC and \MPP from pre-training, which are called \textbf{\method w/o \CGC} and \textbf{\method w/o \MPP} respectively. We name this model that only uses paired sequence and germline as input and optimize MLM on them as \textbf{\method w/o \CGC \& \MPP}.

%\textbf{Architectures and Training}
%\label{setup}
%We use the base Transformer architecture~\citep{vaswani2017attention} with 12 layers, 12 heads and 768 hidden states. The total parameters are 86M. For each tasks in \benchmark, we finetune the model with supervised data. We follow the standard split of Antigen Binding Prediction. For other tasks that do not provide standard split, we conduct 10-cross validation and report the average results. Since our pre-training model learns the representation of the antibody sequence, we expand the CDR fragment to the full antibody via searching the biological database for therapeutic antibody engineering tasks. The training details are attached in Appendix. 


\textbf{Evolution-aware antibody pretraining method} 
To incorporate the biological mechanism into the pre-training, we propose a model with evolution information: \textbf{A}ntibody \textbf{E}volu\textbf{T}ion-aware pretraining \textbf{L}anguage \textbf{M}odel. The antibody can be represented as $A$ and the germline of the individual antibody can be represented as $G$. Typically, PALMs are trained with basic masked language modeling (MLM). Based on it, we design another two pre-training objectives to simulate the biological mechanism of antibody evolution. The evolutionary relationship between the antibody and its germline includes two folds: (i) \textit{Whether the antibody and the germline have an evolutionary relationship}. (ii) \textit{How to mutate residues from the germline to get the specific antibody}. 
Two evolution-related objectives are introduced to solve the above questions: \textbf{Ancestor Germline Prediction (\CGC) }and \textbf{Mutation Position Prediction (\MPP)}. For ancestor germline prediction, we substitute the paired germline $G$ with random germline $G'$ in the batch via a probability $p$. The model is made to distinguish the ancestor germline of the antibody by capturing the shared features.
To predict mutation position, for each token in the germline $G$, the objective is to predict a 0/1 label for each token to indicate whether this token has been mutated. For the antibody sequence $S$, we mask the mutation position and predict these tokens.  

\textbf{Hyper-parameters} We use the base Transformer architecture~\citep{vaswani2017attention} with 12 layers, 12 heads, and 768 hidden states. For each task in \benchmark, we finetune the model with supervised data. We follow the standard split of Antigen Binding Prediction. For other tasks that do not provide a standard split, we use a 10-fold cross-validation. Since our pre-training model learns the representation of the antibody sequence, we expand the CDR fragment to the full antibody by searching the biological database for therapeutic antibody engineering tasks. We also use the same Transformer architecture to train from scratch for each downstream task. This model is indicated as \textbf{non-pretrain} since it is not pre-trained on a protein/antibody database.

\textbf{Reproduction} 
We conduct 10-fold validation on paratope prediction, B cell maturation analysis, and antibody discovery. For antigen binding prediction, we conduct three repetitive experiments with different random seeds. We report the average results and the standard derivation. 
% The benchmark and code will be released. 

% In this section, we first introduce our evolution pre-training framework for antibody, including a germline-context MLM and two antibody-specific training objectives. And then we set up our experiments and introduce baselines.

%\subsection{Evolution-aware Pretraining}
% In order to incorporate the evolutionary information into the pre-training, we pair the antibody sequence $A$ with its germline $G$ and concatenate them into a long sequence with a special token `[SEP]' as the delimiter: $S=\{s_1, \cdots, s_{m+n+1}\}=\{a_1, \cdots, a_m, \text{[SEP]}, g_1, \cdots, g_n\}$. Thus, we optimize MLM objective on the long sequence $S$:
% \begin{align}\small
%     l_{\text{MLM}} = - \frac{1}{|M|} \sum_{i \in M}{\log{p(s_{i} | S_{\backslash M})}},
% \end{align}
% where $M$ is the index set of masked tokens.
% It helps the model to learn the basic residue distribution for antibody sequences. Besides, it can also capture the interaction between residues of the antibody and its germline.

%\begin{figure}[ht]
%    \centering
%    \begin{subfigure}{0.48\textwidth}
%        \includegraphics[width=\textwidth]{figs/model1.pdf}
%        \caption{Pre-training with two biological evolution tasks.}
%        \label{fig:pretain}
%    \end{subfigure}
%    \hfill
%    \begin{subfigure}{0.48\textwidth}
%        \includegraphics[width=\textwidth]{figs/22.pdf}
%        \caption{Finetuning for three biological categories in \benchmark. }
%        \label{fig:finetune}
%    \end{subfigure}
%    \caption{\method. In Figure \ref{fig:pretain}, \CGC randomly unpairs the germline sentence and predict the ancestor relationship. \MPP predicts the mutation position on the germline and the masked mutation residue on the antibody. Based on the input, the three categories in \benchmark can be divided into sequence-level and individual-level (Figure \ref{fig:finetune}). For individual-level disease diagnostics, we score each sequence in the individual profile and calculate the trimmed mean over all sequences to get the individual score.}
%    \label{fig:model}
%\end{figure}


%\textbf{Ancestor Germline Prediction}
%The ancestor relationship between the antibody and its germline determines the shared biological functions obtained in the evolution. Antibody sequences with similar residues evolved from different germline sequences may have different biological functions.
% When stimulated by a foreign antigen, the common ancestor germline evolve to various antibody sequences. Similar antibody sequences may have different germline sequences, which will affect their biological functions. 
%Thus, the aim of this task is to determine whether the antibody have evolutionary relationship with the given germline. 
%During training, we substitute the paired germline $G$ with random germline $G'=\{g_1, \cdots, g_n\}$ in the batch via a probability $p=0.3$. The new sequence is denoted as $S'=\{a_1, \cdots, a_m, \text{[SEP]}, g'_1, \cdots, g'_n\}$ and the training loss can be described as:
%\begin{align}\small
%    l_{a} = - \log{p(y|S')},
%\end{align}
%where $y \in \{0,1\}$ indicate whether the noisy germline $G'$ is the ancestor of the antibody $S$. It can help the model to distinguish the ancestor germline of the antibody by capturing the shared features.


%\textbf{Mutation Position Prediction}
%The somatic hypermutations on the germline further give progeny antibodies the specificity of binding with the specific antigen. In order to model this specificity, this task focus on predicting the mutation positions and the residues mutated to.
%Specifically, for each token $g_j$ in the germline $G$, the target is to predict a label $y_j \in \{0,1\}$ to indicate whether this token has been mutated. For the antibody sequence $S$, we mask the mutation position and predict these tokens. The objective can be formalized as:
%\begin{align}\small
%    l_{m} = - \frac{1}{n} \sum_{j \in \{1,\cdots,n\}}\log{p(y_{j}|S_{\backslash %\end{align}
%Here, $M'$ is the ground-truth mutation position and we mask these tokens on the antibody sequence.
% This task is more difficult than MLM which equally masks tokens in the $L$, because the tokens on the mutation position of $A$ get less  information from the germline, compared with other shared residues between the antibody and the germline. 
%By optimize this objective, the model learn to capture the specificity obtained from the somatic hypermutation in the evolutionary process.





% We use Adam optimizer~\citep{kingma2015adam} with the maximum learning rate of 2e-4 and the warm-up step of 24,000. The maximum length is set to 400 since most antibody sequences are shorter than 180. We first pre-train our model with MLM objective. During the pre-training, 15\% tokens are randomly selected with 80\% masked, 10\% replaced and 10\% kept.  Then we conduct further pre-training on two evolution-related tasks with a smaller learning rate of 1e-5. The model is trained with 108,000 steps and get 0.9606 token accuracy on MLM task. It takes further 72,000 steps for \CGC and \MPP, and obtain 0.4430 token accuracy in mutation position prediction. 



% Pretraining language models with huge unsupervised data and large neural network architecture have been applied to learning informative representation for protein and antibody sequences. 
% Existing work view the biological sequence as the natural language sequence and use the MLM as the training objective~\citep{elnaggar2021prottrans,rives2021biological,ruffolo2021deciphering,leem2021deciphering}. 
%\citet{olsen2022ablang} train antibody pretraining language models based on Transformer~\citep{vaswani2017attention} on the OAS database to optimize MLM objective. A heavy chain version \textbf{Ablang-H} is trained on 14M sequences and A light chain version \textbf{Ablang-L} on 0.19M sequences. \textbf{ESM-1b}~\citep{rives2021biological} is a protein language model that is trained on 250M protein sequences of the Uniparc database~\citep{bairoch2005universal}. It is also based on Transformer and use MLM as the training objective. For fair comparison,  we use the released base version which has 86M parameters (refer as \textbf{ESM-1}). {MSA-1b}~\citep{rao2021msa} is also a Transformer-based language model which takes MSAs (Multiple Sequence Alignment) as the input to extract context embeddings. Since it is difficult to align sequences between antibodies due to the diversity of CDR3, we take the corresponding germline and create MSAs with depth 2. 

%AntiBERTa~\citep{leem2021deciphering} 
% and AntiBERTy~\citep{ruffolo2021deciphering} both 
%follow the BERT~\citep{devlin-etal-2019-bert} setting to train the antibody language model on OAS. AntiBERTa is trained on 2.3M heavy chain and 15.3M light chain sequences.
% , while AntiBERTy was trained on 588M antibody sequences including both heavy and light chain. 
%Since it has not been released, we train a BERT model on the full OAS database with the 
%same setting, which is named \textbf{AntiBERT}. We also use the same Transformer architecture to train from scratch for each downstream task. This model is indicated as \textbf{Transformer} since it does not have pre-training.






==> [arxiv] Antibody/sections/005discussion.tex <==
In this section, we present the experimental results and analysis for the representation capability of existing PPLMs, PALMs, and the \method method with evolutionary incorporation, using \benchmark benchmark. Additionally, we summarize our observations aiming to address the problems highlighted in the introduction.
% The task description and methods are described in Section \ref{sec:task} and \ref{sec:method}. %Then, we provide an interpretable analysis of the learned evolutionary scope. 

% \begin{wrapfigure}[10]{r}{0.5\linewidth}
%     \vspace{-35pt}
%     \centering
%     \!\!\!\!\!\!\!\includegraphics[width=0.5\textwidth]{figures/grad.pdf}
%     \vspace{-10pt}
%     \caption{Comparison of training process of exact and inexact gradient estimation on WMT14 En-De validation set.}
%     \label{fig:grad}
% \end{wrapfigure}

\subsection{Main Results}

%Comparing Figure \ref{fig:cumsum_t8}, \ref{fig:cumsum_t85} and  \ref{fig:cumsum_t9}, we find the model performance has a similar tendency, but when released the matching requirement, the classifiers do not have many advantages over the random order. 

%Meanwhile, we can find that at the beginning, where the classifiers give the highest score, all models are worst than the expected random baselines. This indicates that the sequences with the highest rank can not match the existing SARS-COV-2 antibody binders. However, the mismatch of most highly rank sequences with the existing binders does not mean that the classifiers have a poor performance, because the database does not cover all possible binders. On the contrary, these sequences show great potential to be a new binder, which can accelerate the process of therapeutic antibody discovery for SARS-COV-2.


\paragraph{Antigen binding} 

We evaluate the performance PLMs models for antibody binding and paratope prediction, which are less antibody specific. The results in Table \ref{tab:specificity} indicate that PPLMs and PALMs perform similarly on these tasks, suggesting that PALMs can learn comparable general protein representations to PPLMs. Among different PALMs, Ablang-H outperforms Ablang-L and AntiBERT. It indicates that separate training for heavy and light chain sequences is beneficial for these tasks. Moreover, the introduction of \CGC and \MPP provides improvement over AUC and F1 metrics.
%Our method \method achieves comparable result with Ablang-H, suggesting evolution information is helpful for the representation. 

\input{tabs/Therapeutic}

\paragraph{Paratope prediction} 

The results presented in Table \ref{tab:specificity} demonstrate that for paratope prediction, both PPLMs and PALMs can significantly boost the prediction accuracy over the model with pre-training. However, PALMs do not exhibit a significant advantage over PPLMs. \method outperforms other models, particularly in terms of F1 and MCC, while other models exhibit high recall and low precision, indicating that they tend to predict more residues as binding sites. With the incorporation of mutation residue prediction, \method can focus on the specific mutated positions adapted to bind with antigen. 
Among the two PPLMs, MSA-1b outperforms ESM-1 on F1 and MCC, which benefits from the structure information learning from MSAs. 
%The potential reason may be the better representation of protein 3D structures derived from MSA-1b can paratope prediction.


%\paragraph{Disease Diagnosis} Disease Diagnosis is an individual-level task whose aim is to discriminate a specific disease from a bag of antibody sequences. Following ~\citet{zaslavsky2022disease}, we considered two steps for the task: first train a sequence-level classifier with noisy labels and use this classifier to get the probability of each sequence in the bag. Then, We calculate the trimmed mean over all sequences to build the Q7 classification task for disease diagnosis. The results of sequence-level classifiers are attached in Appendix, and here we present the individual-level results in Table \ref{tab:disease_q7}. 

%\input{tabs/disease_q7}
%Table 5 show the results of disease diagnosis. We can easily observe that \textit{pre-training strategy doesn't help this task}: all PLMs show comparable or even worse results as random initialized Transformer model. The potential reason could be the sequence noise is very large, and model training mainly depends on the finetune process of the subsequent disease data.

%\input{tabs/cell_analysis}

\begin{wrapfigure}[16]{r}{0.45\linewidth}
    \vspace{-10pt}
     \raggedright 
         \includegraphics[width=0.45\textwidth]{figs/cell.pdf}
          \vspace{-20pt}
         \caption{B cell evolution category prediction. For each $p_{ij}$ in $i-$th row and $j$-th column, it means the frequency for the model to predict the antibody in $i$ category to $j$ category. The number is normalized by row.}
         \label{fig:B_cell}
     % \end{subfigure}
\end{wrapfigure}

\paragraph{B Cell Analysis} 

In this task, we investigate the ability of different pre-trained language models to distinguish between various B cell mature states during evolution.  
The findings, as demonstrated in Table \ref{tab:specificity}, indicate that PPLMs are not effective in discerning minor differences between B cell sequences, resulting in mediocre results.
% The results are shown in Table \ref{tab:specificity}. In general, we find PPLMs can hardly distinguish the minor differences between B cell sequences by showing compromising results. 
Both ESM-1 and MSA-1b perform significantly worse than randomly initialized models. MSA-1b, in particular, performs poorly among all pre-trained language models, implying that representations that excel in protein structure prediction may be detrimental to antibody-specific tasks. 
% Both the performance of ESM-1 and MSA-1b is significantly worse than randomly initialized models. MSA-1b performs the worst in all pre-trained language models, indicating representation that can perform well in protein structure prediction will be harmful to antibody-specific tasks. 
Conversely, all PALMs show promising results for the task. This may be due to the fact that the general protein has little correlation with the specific antibody mature process and cannot capture this feature during protein pretraining. Our \method significantly outperforms the other PALMs. This is because our model can effectively capture the evolution feature and better distinguish between B cells at different stages of maturation by explicitly modeling the biological mechanism.
% The reason may lie in that the general protein has little relationship with the special antibody mature process and can hardly capture this feature during the protein pretraining process.
% \method significantly outperforms the other PALMs. This is because by explicitly modeling the biological mechanism, our model can effectively capture the evolution feature and better distinguish between B cells at different stages of maturation.

We conduct further analysis to figure out whether our \method successfully captures sequence characteristics during the evolutionary process. We explore the probabilities of predicting antibodies in class $i$ to class $j$.
% by classifying B cell sequences into 6 different evolutionary categories. %We randomly select 8000 sequences and demonstrate the prediction result of \method on each category in Table \ref{fig:cell_analysis}. 
%The order of B cell type follows the evolutionary process in the immune system, from immature state to transitional state and finally becomes a memory B cell. Both memory IgD- and IgD+ belong to memory B cells with different isotypes, and they have a high affinity to foreign antigens. Among the other categories, the Plasmacytes PC sequences also have some affinity ability. 
The results shown in Figure \ref{fig:B_cell} reveal \method can easily classify the immature B cell with an accuracy of 0.9. It is consistent with the biological study that CDR3 sequence length in immature B cells is significantly shorter than that of the other mature B cells~\citep{ghraichy2021different}. From the diagonal, we can figure out that our model tends to mistake the B cell sequences with their previous or post-evolutionary stage, consistent with the biological process. 


\paragraph{Antibody Discovery} 


\begin{wrapfigure}[18]{r}{0.45\linewidth}
    \vspace{-10pt}
     \raggedright 
         \includegraphics[width=0.45\textwidth]{figs/SARS_90.pdf}
          \vspace{-20pt}
         \caption{The cumulative sum of matched sequences number in the order of the predicted probability. EATLM outperforms other PALMs and PPLMs for finding SARS-CoV-2 binder faster highlighted in \textcircled{1} and finding all antibodies faster highlighted in \textcircled{2}.}
         \label{fig:t9}
     % \end{subfigure}
\end{wrapfigure}

% We examine PPLMs and PALMS for their capacity in benefiting real-world problems and enabling the discovery of antigen-specific antibodies. Following the methods in this study \citet{zaslavsky2022disease}, we considered two steps for the SARS-CoV-2 specific antibody discovery. 
We investigated the potential of PPLMs and PALMs in aiding the discovery of antigen-specific antibodies for real-world problems. To achieve this, we followed a two-step process similar to \citet{zaslavsky2022disease}.
Firstly, we created a sequence classifier to differentiate SARS-CoV-2 antibodies using noisy individual-level labels. Secondly, we compared the highly-ranked sequences with true binding sequences in the CoV-AbDab~\citep{raybould2021cov} database to determine if there are similarities. 
We used a 90\% sequence identity threshold to determine the likelihood of biological functionality similar to the existing binders. The experimental design for this is outlined in \S \ref{sec:sars_discovery}.
% First, we generate a sequence classifier to distinguish SARS-CoV-2 antibodies using noisy individual-level labels. Then, the high-ranked sequences are matched with the sequences with true binding sequences in the CoV-AbDab~\citep{raybould2021cov} database. %For the first step, we find our evolution-aware EATLM performs the best in the individual-level classifier to determine whether the patient suffering from SARS. Besides, PALMs significantly outperform PPLMs. 
% We use the 90\% sequence identity as the threshold to determine whether the antibody is similar to existing SARS binders in the CoV-AbDab database. A high similarity indicates a high probability of having the same biological functionality as the existing binders. The experimental setup is in \S \ref{sec:sars_discovery}. 


% In Figure \ref{fig:t9}, we plot the cumulative sum of matched sequences number in the order of the predicted probability of the classifiers. 
Figure \ref{fig:t9} shows the cumulative sum of matched sequences in the order of predicted probabilities by different pre-trained language models for the SARS-CoV-2 specific antibody discovery task.
% We can observe that the sequences predicted with high probability by PALMs match with the existing binders better than PPLMs. It means that PALMs can figure out the potential binders more efficiently.
We can observe that PALMs outperform PPLMs in identifying potential binders, as the sequences predicted with high probability by PALMs match better with the existing binders. 
Moreover, among PALMs, \method significantly outperforms other models, with the red line indicating its performance. Initially, \method is the quickest method to find potential binders, but it loses to Ablang-H, and eventually overtakes again and converges. This suggests that \method is the most effective method for identifying all potential binders in this dataset.
% Besides, \method significantly outperforms other PALMs as the red line shows. In the early stage, this method is the quickest way to find potential binders. Then it loses to Ablang-H but finally overtakes again and converges. It means that \method is the first one to figure out all potential binders in this dataset.


%  \begin{wrapfigure}[10]{r}{0.5\linewidth}
%     \vspace{-35pt}
%     \centering
%     \!\!\!\!\!\!\!\includegraphics[width=0.5\textwidth]{figs/SARS_90.pdf}
%     \vspace{-10pt}
%     \caption{Comparison of training process of exact and inexact gradient estimation on WMT14 En-De validation set.}
%     \label{fig:grad}
% \end{wrapfigure}

Furthermore, we list 11 potential binder sequences discovered by \method in Table \ref{tab:11binder}. Without supervised labels, \method gives a high probability of 2 SARS-CoV-2 existing binding antibodies. Besides, \method suggests 9 potential sequences with high CDR-H3 sequence identity, indicating the potential for diverse-epitope antibody discovery and selection. 
% Further analysis of the results reveals that \method enables diverse-epitope antibody discovery and priority selection, demonstrating that \method benefits therapeutic antibody discovery.
These results demonstrate the potential of \method in therapeutic antibody discovery.

To validate whether the antibody sequences with 90\% sequence identity can indeed bind the same target, we investigate the 3D structure of the true binding antibody. Table \ref{fig:3d_binder} shows only one single residue difference between the predicted binder and the existing binder, suggesting the predicted binders are highly possible to interact with SARS-CoV-2. 



%\input{tabs/task}
% \input{tabs/newbinder}
\input{tabs/discovery.tex}  


% \end{figure}



 


%\subsection{Discussion}

%\textbf{Germline Visualization} First, we wonder whether the model learns the shared biological features between the antibody and its ancestor germline?
%To answer this question, we select two profiles with a comparable number of antibody sequences either from healthy and SARS-COV-2 infected individuals and visualize the sequences with different germlines using UMAP analysis in Figure \ref{fig:germ_health} and \ref{fig:germ_sars}. We found for both the health profile and the patient, antibodies evolved from the same germline are nicely clustered together, indicating the learned embedding is encoded with germline information.

%Sequences derived from germline 1 and 6 show similar representations in Figure \ref{fig:germ_health}, which may due to the high sequence similarity between their germlines. 

% Then, we group the antibody sequences in each profile using germline v gene labels. The germline groups that have less than 100 sequences are removed. UAMP visualization analysis is conducted for antibody sequence with different germline labels in Figure \ref{fig:germline}. We find that the representations encode the germline information and gather sequences with the same germline together. However, in Figure \ref{fig:germ_health}, there are also sequences of different germlines that are similar in representation, such as germline groups 1 and 6, which may be caused by similarity in their germline sequences. Compared with it, Figure \ref{fig:germ_sars} has fewer germline groups and the sequence representations are more discrete in the UMAP space. This phenomenon fits well with the immune response, where little germlines are stimulated and evolute to antibody sequences with affinity to SARS-CoV-2 by somatic hypermutation. Thus the representation of antibody sequences that undergo huge mutation are scattered from each other but still cluster around the same germline.



%\textbf{Evolutionary Distance} Second, we ask whether the representation can reflect the evolutionary distance between the antibody and its ancestor germline? We adopt the same two profiles as above and plot the evolutionary distance using heat bar (Figure \ref{fig:health_dist} and \ref{fig:sars_dist}). Interestingly, sequences with similar scales of evolutionary distance tend to cluster together, and a clear gradation of evolutionary distance can be observed in Figure \ref{fig:sars_dist}. These results indicate that our representation can efficiently capture the evolutionary distance. 

%sequences and their germline in Figure \ref{fig:dist}. We color the antibody with its evolutionary distance with its germline. The distance for the germline itself is 0. From Figure \ref{fig:health_dist} we can find that sequences with the same shades are usually clustered together. Besides, the shades of color have a gradation in space, which is more obvious in Figure \ref{fig:sars_dist}. It indicates the distances in the UMAP space are consistent with the evolutionary distances, which proves that our representation can reflect the evolutionary distance.





% \begin{figure}[h]
%     \centering
%         \includegraphics[width=\textwidth]{figs/Figure4.pdf}
%     \caption{The cumulative count of matched sequences number. The dashed line is the expected results for a random order. The x-axis is the sequence number and the y-axis is the cumulative matched sequence number.}
%     \label{fig:cumsum}
% \end{figure}

%\textbf{SARS Antibody Discovery} Antibody discovery from B cell repertoire has been widely recognized as a novel trend to improve the efficiency of antibody discovery for diverse antigens ~\citep{weiner2015building,pedrioli2021single}. Here, we ask whether PLMs can benefit real-world problems and enable fast-track neutralization SARS-CoV-2 antibody discovery. The task is highly challenging from two aspects: (1) Less than 1\% of antibodies from SARS-CoV-2 patients are directly responsible for virus binding. (2) It is hard to get a reliable sequence-level classifier using unreliable and noisy individual-level labels. The detailed result of our sequence classifier can be found in Appendix. Following the methods in this study \citet{zaslavsky2022disease}, we match the high-ranked sequences with the sequences in the Cov-AbDab~\citep{raybould2021cov} database, which have been proved to bind SARS-CoV-2 using wet-lab experiments. Notably, as shown in the appendix, \method find 2 SARS-CoV-2 true binding antibodies and 35 likely sequences matched with high CDR-H3 sequence identity (over 85\%). Further analysis of the results reveals \method enable diverse-epitope antibody discovery and priority selection, demonstrating \method can be useful for therapeutic antibody discovery. 

%To quantitatively compare with others, we plot the cumulative sum of matched sequences number in the order of the predicted probability of the classifiers. Figure \ref{fig:cumsum} shows the results of different models under different identity thresholds for the match with the Cov-AbDab database. In general, PLMs are useful for this task and antibody-specific PLMs, our \method and Ablang-H significantly outperforms other PLMs. In the early stage, \method outperforms other models and starts to beat the expected results. Then it loses to Ablang-H but finally overtakes again and becomes the first to converge. This result indicates, compared with other approaches, \method can more efficiently capture the true binders from noisy sequences. Comparing Figure \ref{fig:cumsum_t8}, \ref{fig:cumsum_t85} and  \ref{fig:cumsum_t9}, we find the model performance has a similar tendency, but when released the matching requirement, the classifiers do not have many advantages over the random order. 

%Note that our sequence classifiers are trained with noisy pseudo labels and do not have any clean labels. The details can be found in Appendix. we plot the cumulative sum of matched sequences number in the order of the predicted probability of the classifier. Figure \ref{fig:cumsum} shows the results of different models under different identity thresholds for the match with the SARS-COV-2 database. 

%In the early stage, \method outperforms other models and starts to beat the expected results. Then it loses to Ablang-H but finally overtakes again and becomes the first to converge. This indicates that \method has the highest consistency with the true binders in highly ranked sequences and can spend less time figuring out all binders. Comparing Figure \ref{fig:cumsum_t8}, \ref{fig:cumsum_t85} and  \ref{fig:cumsum_t9}, we can find the model performance has a similar tendency, but when released the requirement for matching, the classifiers do not have many advantages over the random order. 

%Meanwhile, we can find that at the beginning, where the classifiers give the highest score, all models are worst than the expected random baselines. This indicates that the sequences with the highest rank can not match the existing SARS-COV-2 antibody binders. However, the mismatch of most highly rank sequences with the existing binders does not mean that the classifiers have a poor performance, because the database does not cover all possible binders. On the contrary, these sequences show great potential to be a new binder, which can accelerate the process of therapeutic antibody discovery for SARS-COV-2.


%\textbf{Disease Diagnosis} Disease Diagnosis is an individual-level task whose aim is to discriminate a specific disease from a bag of antibody sequences. We use all these diseases profile to build the Q7 classification task for disease diagnosis. Previous biological studies mainly use this multi-classification task for disease diagnosis ~\citet{zaslavsky2022disease,wang2022large}, highlighting the discriminatory power among different diseases are important for disease diagnosis. Following the practice of \citet{zaslavsky2022disease}, we first train a sequence-level classifier with noisy labels and use this classifier to get the probability of each sequence in the bag. Then, We calculate the trimmed mean over sequences to get a final probability as the score for this individual. The results of sequence-level classifiers are attached in Appendix, and here we present the individual-level results in Table \ref{tab:disease_q7}. 

%\input{tabs/disease_q7}
%Table 5 show the results of disease diagnosis. First, we can easily observe that pre-training is not important for this task: all PLMs show comparable or even worse results as random initialized Transformer model. The potential reason could be the sequence noise is very large, and model training mainly depends on the finetune process of the subsequent disease data.



%\begin{figure}
%     \centering
%     \begin{subfigure}{0.49\textwidth}
%         \includegraphics[width=\textwidth]{figs/health.freq1000.pdf}
%         \caption{Health profile.}
%         % \vspace{-0.5\baselineskip}
%         \label{fig:health_dist}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \includegraphics[width=\textwidth]{figs/sars.freq1000.pdf}
%         \caption{Patient profile.}
         % \vspace{-0.5\baselineskip}
%         \label{fig:sars_dist}
%     \end{subfigure}
%     \caption{UMAP Visualization for evolution phylogeny distance. The shade of color indicate its distance from the ancestor germline.}
%     \label{fig:dist}
% \end{figure}

%\begin{figure}[h]
%    \centering
 %   \begin{subfigure}{0.36\textwidth}
%        \includegraphics[width=\textwidth]{figs/model.cdrmatch.top10000.t8.pdf}
%        \caption{Threshold=0.8}
%        \label{fig:cumsum_t8}
%    \end{subfigure}
%    \hspace{-8mm}
    % \hfill
 %   \begin{subfigure}{0.36\textwidth}
%        \includegraphics[width=\textwidth]{figs/model.cdrmatch.top10000.t85.pdf}
%        \caption{Threshold=0.85}
 %       \label{fig:cumsum_t85}
%    \end{subfigure}
%    \hspace{-8mm}
    % \hfill
%    \begin{subfigure}{0.36\textwidth}
%        \includegraphics[width=\textwidth]{figs/model.cdrmatch.top10000.t9.pdf}
%        \caption{Threshold=0.9}
%        \label{fig:cumsum_t9}
%    \end{subfigure}
%    \caption{The cumulative count of matched sequences number. The dashed line is the expected results for a random order. The x-axis is the sequence number and the y-axis is the cumulative matched sequence number.}
%    \label{fig:cumsum}
%\end{figure}



%\textbf{Answer for Q(1): Yes.} Antibody PLMs can learn biologically meaning representations. However, more comprehensive pretraining objectives are needed to help PLMs to learn antibody representations better. Futher studies in this direction could be very interesting.

%\textbf{Answer for Q(2): Yes.} Both antibody PLMs and protein PLMs are helpful for majority of antibody prediction tasks, except disease diagnosis. One of the potential reason underlying the limited performance could be the complexity of disease diagnosis.

%\textbf{Answer for Q(3): It depends on the downstream tasks.} For tasks more antibody-specific evolution information required, like B Cell analysis and antibody discovery, antibody PLMs significantly outperform protein PLMs. While for the therapeutic antibody engineering, a task less evolution information related, antibody PLMs does not obviously outperform protein PLMs.

%\textbf{Answer for Q(4): Yes. Antibody evolution aware PLM is helpful for antibody prediction tasks, especially the tasks evolution are rela
\vspace{-35pt}
\subsection{How does evolution pretraining task influence the representation?}
To comprehend the reasons for the better performance of \method on antibody-related tasks, we conduct the analysis of the pre-trained representations. The objective of this analysis is to evaluate the effectiveness of the evolution-aware pre-training strategies from two perspectives: (1) Does the pre-trained representation of antibodies reflect their ancestor relationship? (2) Does the specificity of antibodies get captured by the evolution objective?
% To understand why \method shows better performance on antibody tasks, we analyze the pre-trained representations to evaluate the effectiveness of the evolution-aware pretraining strategies from two aspects: (1) Does the pre-trained antibody representation reflect its ancestor relationship? (2) Is the specificity of antibodies captured by the evolution objective?
% In general, \method is more efficient than other PALM in learning antibody-specific characteristics. 

%In general, both strategies are useful allowing PLMs to effectively learn evolutionary relationships. \textbf{}
%\subsection{\textbf{Q(1): Antibody-specific PLMs significantly outperform protein58PLMs for antibody tasks, suggesting general protein pretrained models are not sufficient in antibody-59 specific representation learning.

%\textbf{pretraing results} Here, we examine the pretraining task results for PLMs to evaluate the effectiveness of the pretraining strategies: (1) taking antibody and germline concatenated sequences as input and (2) antibody evolution-specific objectives. In general, both strategies are useful allowing PLMs to effectively learn evolutionary relationships. 

\paragraph{Ancestor Gerlime Visualization} We perform UMAP visualization analyses in Figure \ref{fig:4germline}. First, we observe that antibodies evolved from the same germline are nicely clustered together (Figure \ref{fig:germ_health} and \ref{fig:germ_sars}), indicating the learned embedding is encoded with germline information. Besides, sequences with similar scales of evolutionary distance tend to cluster together, and a clear gradation of evolutionary distance can be observed in Figure \ref{fig:health_dist} and \ref{fig:sars_dist}. The visualization provides a sanity check for the ability of EATLM to extract the sequence information of antibodies.

\paragraph{Accuracy of Mutation Position} 
Based on the specific evolution process described in \S \ref{sec:background}, we can find the mutation during the evolution process bring specificity to the antibody. Thus, we explore the model's ability to predict mutated residue from the masked token, which can reflect the specificity feature the model captures. We find that although AntiBERT can predict with an accuracy of 0.889 on all positions, it fails on mutation positions with a 0.031 accuracy. In contrast, \method achieves an accuracy of 0.443 on mutation position, which indicates that the model captures the specificity information. Note that during the \MPP training, we mask the mutation position on antibody sequences, which are different from its germline. Thus, the model cannot get the mutated residue from the germline directly. The only way is to learn the underlying mutation rules. The full results are shown in Table \ref{tab:pretrain} in Appendix.



%Due to the high sequence similarity between antibody with its germline, EATLM taking concatenated sequence as input can easily predict the ancestor germline and mutation position by self-attention between antibody and germline. On the contrary, AntiBERT, without concatenating germline sequence as input, is difficult to predict the ancestor relationship. Notably, removing the evolution-related objectives from the pretraining results significant decreased accuracy of mutation positions to 0.0311 and 0.8889 on all positions. 
%For mutation amino acid prediction, EATLM only obtained 0.4430 accuracy. We assume it is because the ancestor germline can undergo different somatic hypermutations and get various progeny antibodies, resulting in different valid mutations at the same position. 
%\input{tabs/Pretrained_2}


%\textbf{Evolutionary representation visualization} Here, take EATLM as an example, we visualize the sequence representation and found PLMs can capture biologically meaningful evolutionary features between the antibody and its ancestor germline. 

%In Figure 2, UMAP visualization analyse was performed to investigate two profiles either from health and patient with comparable number of antibody sequences. It is observed antibodies evolved from the same germline are nicely clustered together, indicating the learned embedding is encoded with germline information. Then, we ask whether the representation can reflect the evolutionary distance between the antibody and its ancestor germline? Evolutionary distance using heat bar is plotted (Figure \ref{fig:health_dist} and \ref{fig:sars_dist}). Interestingly, sequences with similar scales of evolutionary distance tend to cluster together, and a clear gradation of evolutionary distance can be observed in Figure \ref{fig:sars_dist}. 

\begin{figure}[ht]
    \centering
    \vspace{-5pt}
    \begin{subfigure}{0.27\textwidth}
        \includegraphics[width=\textwidth]{figs/health.germtype.pdf}
        \caption{Health germlines.}
        \label{fig:germ_health}
    \end{subfigure}
    % \hfill
    \hspace{-7mm}
    \begin{subfigure}{0.27\textwidth}
        \includegraphics[width=\textwidth]{figs/sars.germtype.pdf}›
        \caption{Patient germlines.}
        \label{fig:germ_sars}
    \end{subfigure}
    % \vskip 0.1\baselineskip
    \hspace{-4mm}
    \begin{subfigure}{0.27\textwidth}
        \includegraphics[width=\textwidth]{figs/health.freq1000.pdf}
        \caption{Health distance.}
        % \vspace{-0.5\baselineskip}
        \label{fig:health_dist}
    \end{subfigure}
    % \hfill
    \hspace{-8mm}
    \begin{subfigure}{0.27\textwidth}
       \includegraphics[width=\textwidth]{figs/sars.freq1000.pdf}
        \caption{Patient distance.}
        % \vspace{-0.5\baselineskip}
        \label{fig:sars_dist}
    \end{subfigure}
    \caption{UMAP Visualization. (a-b) for sequences with different germlines. One color indicates one germline with its descendant. (c-d) for evolutionary phylogeny distance. The shade of color indicates its distance from the ancestor germline.}
    \label{fig:4germline}
\end{figure}


\subsection{Key Observations}

\textbf{The performance of pre-trained language models is highly dependent on the specificity of the task.}  In tasks with low antibody-specificity, PPLMs perform similarly to PALMs, indicating that using general protein representations from PPLMs is an effective way to transfer learning in these tasks. On medium specificity tasks such as paratope prediction, PALMs show their advantage and outperform PPLMs. However, for tasks with high specificity, PPLMs have significantly lower performance, suggesting that general pre-trained protein models are insufficient for antibody-specific representation learning. Additionally, incorporating protein evolution information does not always benefit antibody tasks, especially those that require antibody evolution information, as shown by the 20\% decrease in performance observed with MSA-1b compared to the model without pre-training. 
% This observation is consistent with the biological study that the mechanism of antibody evolution is significantly different from that of proteins.
This finding is consistent with the biological understanding that the mechanism of antibody evolution is significantly different from that of proteins.
% Therefore, the incorporation of protein evolution information is not always good for antibody tasks, especially the tasks that require antibody evolution information.
% , which is beneficial for protein structure prediction, is harmful to antibody evolution-specific tasks.

 \begin{wrapfigure}[12]{r}{0.4\linewidth}
     \vspace{-30pt}
      \raggedright 
          \includegraphics[width=0.4\textwidth]{figs/specificity.pdf}
           \vspace{-25pt}
          \caption{Performance summary of various pre-trained language models.}
          \label{fig:task}
      % \end{subfigure}
\end{wrapfigure}
\textbf{Incorporation of biological evolution mechanism into PALM generally benefits antibody prediction tasks.} 
The inclusion of evolution-related training objectives assists in identifying mutation positions on antibodies, which is a distinguishing feature from germline. 
% Evolution-related training objectives help detect mutation positions on antibodies, which is a distinguishing feature from germline. 
% Table in Appendix \ref{fig:pretain} shows removing the evolution-related objectives from pretraining results in significant decrease accuracy of mutation ?prediction from 0.443 to 0.0311. 
% Downstream task performance results can be found in Figure 3 and Table 3, showing antibody evolution-aware PALM outperforms the other PALMs as well as PPLMs in three antibody prediction tasks. 
Notably, the performance increase of \method in comparison to other PALMs is linked with the level of task specificity. The ablation study showed removing the evolution-related pretraining objectives leads to decreased performance, confirming their contribution to the prediction task. Further research in this direction is promising and could offer more in-depth insights.
% Interestingly, the performance increase of \method compared with other PALMs is correlated with task specificity relatedness. The ablation study showed the removal of the evolution-related pretraining objectives results in performance decreasing, confirming that evolution-related objectives benefit the prediction. Future studies to have more in-depth research in this direction could be promising. %Together with the ablation study, we conclude that \textbf{ evolution-aware antibody-specific PLM can significantly improve the effectiveness for antibody representation learning. }

\textbf{Antibody pre-trained representations are helpful for real-world drug discovery.} By utilizing the language model, we predict the likelihood of each antibody binding with SARS-CoV-2. Despite lacking precise sequence-level labels, we successfully identify 11 promising antibody binders.
% Using the language model, we predict the probability for each antibody of being a binder with SARS-CoV-2. Without accurate sequence-level labels, we successfully identify 11 potential antibody binders.



% \input{tabs/case_study.tex}

% \input{tabs/discovery.tex}

==> [arxiv] Antibody/sections/007conclusion.tex <==
In this paper, we conduct a detailed investigation into the effects of pre-trained protein and antibody language models on various antibody tasks. To facilitate research in the antibody and machine learning fields, we provide \benchmark consisting of four important antibody tasks from four different biological categories with varying levels of antibody specificity.

% In this paper, we have presented comprehensive empirical studies to characterize the impact of pre-trained protein and antibody language models for antibody prediction tasks. Four important antibody tasks from four biological categories with evolution relatedness ranging from high to low are provided \benchmark to facilitate the antibody and ML field. 
%We draw several important conclusions: (1) PLMs are generally important for antibody prediction. (2) Antibody-specific PLMs outperforms protein PLMs for high evolution-related tasks. (3) Interesting, modeling antibody evolution can generates better representation on the high evolution-related tasks. Future studies further explore evolutionary scope may have great promise in antibody representation and prediction. 

%In this paper, we propose \method that incorporates evolution information into the antibody representation learning from the sequence-level ancestor relationship and residue-level mutation modeling. We also benchmark six important antibody tasks from three biological categories and provide \benchmark to facilitate the antibody field. \method achieve satisfying results on the benchmark and further analysis proves that the learned evolutionary scope shows great promise in antibody evolution understanding and SARS-CoV-2 antibody discovery.

However, there are certain constraints to our research. Firstly, due to the scarcity of data, the diversity of tasks in our \benchmark is limited. As more data becomes available, we anticipate expanding our benchmark to include a greater range of diseases and larger data sets. 
Additionally, we did not examine any 3D structure information during antibody pre-training. As antibody structures offer more information than just sequences, such as geometry, incorporating structural information in future studies may lead to improved results.


% However, there are some limitations to this work. First, for the \benchmark , the task diversity is highly limited because of data scarcity. With the data increase in this field, we expect we can update our benchmark with more disease diversity and data size in the future. 
%Also, some studies reported that many biological and clinical factors, such as age, gender, genetic background, and preexisting conditions, are associated with disease diagnosis. Detailed analysis of the impact of different biological factors on model performance would be interesting. 
% Also, we do not test any 3D structure information during antibody pre-training. As a special subgroup of proteins, antibody structures provide much more information such as geometry than sequences. In the future, recruiting structure information for antibody pre-training may be able to improve the results. 


==> [arxiv] Antibody/sections/acknowledge.tex <==
We thank members of ByteDance Research for discussion, Zaixiang Zheng and Yi Zhou for useful writing suggestions. Hao Zhou is supported by Vanke Special Fund for Public Health and Health Discipline Development, Tsinghua University (NO.20221080053), Guoqiang Research Institute General Project, Tsinghua University (No. 2021GQG1012);

==> [arxiv] Antibody/sections/checklist.tex <==

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> [arxiv] Antibody/sections/ethic.tex <==
This research involving the use of pre-existing data and computational methods did not involve any human or animal subjects, and therefore, no ethical approval was required. The authors followed all applicable ethical standards and guidelines for data analysis and reporting. All data used in this study were obtained from publicly available sources, and proper citation and attribution have been given. The authors have made efforts to ensure that the research presented in this paper does not infringe upon any existing copyrights or intellectual property rights.

==> [arxiv] Antibody/tabs/ESMFT.tex <==
% Table generated by Excel2LaTeX from sheet 'BCR'
\begin{table}[htbp]
  \centering\footnotesize
  \setlength{\tabcolsep}{2pt}
  \caption{The performance of larger models and finetuned protein language models on three tasks. The ESM-1 and ESM-1b models have 85M and 650M respectively. The \method-large have similar architecture with ESM-1b. `FT' indicates the model is further finetuned on our antibody pre-training dataset.}
  \label{tab:esmft}%
    \begin{tabular}{lrrrrrr}
    \toprule
    & \multicolumn{3}{c}{\textbf{Antigen Binding}} & \multicolumn{3}{c}{\textbf{Paratope}} \\
    \cmidrule{2-7}      
    & \multicolumn{1}{c}{\textbf{ AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{ AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}}  \\
    \midrule
    ESM-1 & 0.917+0.001 & 0.854+0.002 & 0.689+0.002 & 0.886+0.009 & 0.669+0.024 & 0.547+0.026  \\
    ESM-1 FT & 0.914+0.001 & 0.858+0.001 & 0.695+0.003 & 0.883+0.009 & 0.657+0.031 & 0.534+0.030 \\
    ESM-1b & \textbf{0.924+0.002} & 0.860+0.002 & \textbf{0.707+0.003} & 0.873+0.009 & 0.655+0.042 & 0.524+0.036  \\
    ESM-1b FT & 0.916+0.003 & 0.844+0.003 & 0.686+0.004 & 0.869+0.010 & 0.660+0.021 & 0.527+0.015 \\
    \midrule
    \method & 0.922+0.052 & \textbf{0.862+0.021} & 0.699+0.027 & 0.887+0.008 & \textbf{0.698+0.017} & \textbf{0.575+0.024}  \\
    \method-large & 0.921+0.004 & 0.854+0.004 & 0.677+0.010 & \textbf{0.887+0.007} & 0.685+0.015 & 0.561+0.020 \\
    \bottomrule
  \end{tabular}%
  
\end{table}%

% \begin{table}[htbp]
%   \centering\footnotesize
%   \setlength{\tabcolsep}{2pt}
%   \caption{The performance of larger models and finetuned protein language models on three tasks. The ESM-1 and ESM-1b models have 85M and 650M respectively. The \method-large have similar architecture with ESM-1b. `FT' indicates the model is further finetuned on our antibody pre-training dataset.}
%   \label{tab:esmft}%
%     \begin{tabular}{lrrrrrrr}
%     \toprule
%     & \multicolumn{3}{c}{\textbf{Antigen Binding}} & \multicolumn{3}{c}{\textbf{Paratope}} & \textbf{Disease Q7} \\
%     \cmidrule{2-8}      
%     & \multicolumn{1}{c}{\textbf{ AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{ AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{ACC}}  \\
%     \midrule
%     ESM-1 & 0.917+0.001 & 0.854+0.002 & 0.689+0.002 & 0.886+0.009 & 0.669+0.024 & 0.547+0.026 & 0.757+0.016 \\
%     ESM-1 FT & 0.914+0.001 & 0.858+0.001 & 0.695+0.003 & 0.883+0.009 & 0.657+0.031 & 0.534+0.030 & \textbf{0.762+0.024}\\
%     ESM-1b & \textbf{0.924+0.002} & 0.860+0.002 & \textbf{0.707+0.003} & 0.873+0.009 & 0.655+0.042 & 0.524+0.036 & 0.692+0.036  \\
%     ESM-1b FT & 0.916+0.003 & 0.844+0.003 & 0.686+0.004 & 0.869+0.010 & 0.660+0.021 & 0.527+0.015 & 0.690+0.029  \\
%     \midrule
%     \method & 0.922+0.052 & \textbf{0.862+0.021} & 0.699+0.027 & 0.887+0.008 & \textbf{0.698+0.017} & \textbf{0.575+0.024} & 0.756+0.020  \\
%     \method-large & 0.921+0.004 & 0.854+0.004 & 0.677+0.010 & \textbf{0.887+0.007} & 0.685+0.015 & 0.561+0.020 & 0.743+0.020  \\
%     \bottomrule
%   \end{tabular}%
  
% \end{table}%


==> [arxiv] Antibody/tabs/PLMs.tex <==
% Table generated by Excel2LaTeX from sheet 'New binder'

\begin{table}[htbp]\footnotesize
  \setlength{\tabcolsep}{2pt}
  \centering
  \caption{Pre-training language models for protein and antibody. Evolution denotes whether evolutionary-related sequences are used during the pretraining. MLM is masked language modeling pretraining objective. HC, antibody heavy chain; LC, antibody light chain.} 
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{ccccccccc}
    \toprule
%     & \textbf{Model}  & \textbf{Param} & \textbf{Dataset} & \textbf{Evolution} & \textbf{Loss} & \textbf{Antibody Tasks} \\ 
%    \midrule
%    \multirow{3}{*}{PPLM} 
%    & ESM-1   & 86M & UniRef50 (27M) & $\times$ & MLM &/ \\
%    & ESM-1 FT  & 86M & UniRef50 + OAS & $\times$ & MLM &/ \\
%    %& ESM-1b  & 1280 & 33 & 650M & UniRef50 (27M seqs) & No & MLM & / \\
%    %& ESM-1b FT & 1280 & 33 & 650M & UniRef50 (27M seqs) & No & MLM & / \\
%    & MSA-1b & 100M & UniRef50 (26M MSAs) & \checkmark & MLM & / \\
%    \midrule
%    \multirow{4}{*}{PALM} 
%    & Ablang-H & 86M & OAS(14M HC) & $\times$ & MLM & Reconstruction \\
%    & Ablang-L  & 86M & OAS(0.19M LC) & $\times$ & MLM & Reconstruction \\
%    & AntiBERTa  & 86M & OAS(72M) & $\times$ & MLM & Paratope Prediction\\
%    & EATLM & 86M & OAS(20M) & \checkmark & MLM,AGP,MPP & ATUE \\
%    %& \textbf{EATLM-large} & 1280 & 33 & 650M & OAS(20M seq) & Yes & MLM,AGP,MPP & \textbf{ATUE} \\
%    \bottomrule
%    \end{tabular}%
    \textbf{Model}  & \textbf{Category} & \textbf{Dataset}  & \textbf{Evolution}  & \textbf{Objective} & \textbf{Antibody Tasks} \\ 
    \midrule
    ESM-1~\citep{rives2021biological} & PPLM  & UniRef50 (27M)  & $\times$ & MLM & - \\
    % Low &  ESM-1 FT & PPLM  & UniRef50 + OAS  & MLM & - \\
    %& ESM-1b  & 1280 & 33 & 650M & UniRef50 (27M seqs) & No & MLM & / \\
    %& ESM-1b FT & 1280 & 33 & 650M & UniRef50 (27M seqs) & No & MLM & / \\
    MSA-1b~\citep{rao2021msa} &  PPLM & UniRef50 (26M MSAs) &  \checkmark & MLM & - \\
    \midrule
    Ablang-H~\citep{olsen2022ablang} &  PALM  & OAS (14M HC)  & $\times$ & MLM & Reconstruction \\
    Ablang-L~\citep{olsen2022ablang}  &  PALM  & OAS (0.19M LC) & $\times$ & MLM & Reconstruction \\
    AntiBERTa~\citep{leem2021deciphering}  & PALM  & OAS (72M)  & $\times$ & MLM & Paratope Prediction \\
    \midrule
    EATLM & PALM & OAS (20M)  & \checkmark & MLM, AGP \& MPP & ATUE  \\
    %& \textbf{EATLM-large} & 1280 & 33 & 650M & OAS(20M seq) & Yes & MLM,AGP,MPP & \textbf{ATUE} \\
    \bottomrule
    \end{tabular}%
    }%
  \label{tab:PLMs}%
\end{table}%




==> [arxiv] Antibody/tabs/Pretrained_2.tex <==
% % Table generated by Excel2LaTeX from sheet 'Pretrained'
% \begin{table}[htbp]
%   \centering
%   \caption{Pretrained Model}
%     \begin{tabular}{lrr}
%     \toprule
%     \textbf{Model} & \multicolumn{1}{c}{\textbf{Loss}} & \multicolumn{1}{c}{\textbf{Step}} \\
%     \midrule
%     % BERT & 0.437 & 568000 \\
%     % BERT + contrastive & 0.558 & 19000 \\
%     % BERT + mutation & 1.744 & 134000 \\
%     EALM w/o \MPP \& \CGC  & 0.143 & 108000 \\
%     EALM w/o \CGC & 1.744 & 134000 \\
%     EALM w/o \MPP & 0.001 & 18000 \\    
%     EALM  & 1.856 & 54000 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:pretrain}%
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Pretrained'
\begin{table}[htbp]\footnotesize
  \centering
  \caption{The pretraining details for different models. The `Germline' is the prediction accuracy of \CGC, and the `Position' and `Mutation' are the accuracy of mutation positions and the mutated residues respectively.}
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Size}}& \multicolumn{1}{c}{\textbf{Loss}} & \multicolumn{1}{c}{\textbf{Step}} & \textbf{Germline} & \textbf{Position} & \textbf{Mutation} \\
    \midrule
    AntiBERT & 85M & 0.437 & 568000 & / & / & / \\
    AntiBERT w \CGC & 85M& 0.558 & 587000 & 0.330 & / & / \\
    AntiBERT w \MPP & 85M& 1.744 & 622000 & / & 0.965 & 0.410 \\
    %\midrule
    %ESM-1 FT & 85M& 0.2636 & 136000 & / & / & / \\
    %ESM-1b FT & 650M & 0.2704 & 278000 & / & / & / \\
    %\midrule
    \midrule
    \method w/o \CGC \& \MPP & 85M& 0.143 & 108000 & / & / & / \\
    \method w/o \CGC & 85M& 1.744 & 134000 & / & 1.000 & 0.443 \\
    \method w/o \MPP & 85M& 0.001 & 126000 & 1.000 & / & / \\
    \method  & 85M & 1.856 & 252500 & 0.9960 & 1.000 & 0.443 \\
    %\midrule
    %\method-large w/o \CGC \& \MPP & 650M & 0.149 & 193000 & / & / & / \\
    %\method-large w/o \CGC & 650M & 1.753 & 267000 & / & 1.000 & 0.438 \\
    %\method-large w/o \MPP & 650M & 0.001 & 200000 & 1.000 & / & / \\
    %\method-large & 650M & 1.773 & 384000 & 0.996 & 1.000 & 0.431 \\
    \bottomrule
    \end{tabular}%
  \label{tab:pretrain}%
\end{table}%



==> [arxiv] Antibody/tabs/QM9.tex <==
% Table generated by Excel2LaTeX from sheet 'QM9'
\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{2.8pt}
  \centering
 \tabcolsep 3pt
\caption{MAEs of targets on QM9.}
    \begin{tabular}{lcccccccccccc}
    \toprule
    \textbf{Models} & $\mu(D)$ & $\alpha$($a^3_0$) 
    & $\varepsilon_\text{HOMO} $   &  $\varepsilon_\text{LUMO} $ 
    & $\Delta\varepsilon $ & $\langle R^2 \rangle (a_0^3)$ &
    ZPVE   & \textit{$U_0$}  &
    \textit{U} & \textit{H}  &
    \textit{G}   & $C_v(\frac{\text{cal}}{\text{molK}})$ \\ 
    \midrule
    \multirow{1}[0]{*}{MXMNet} & 0.0396 & 0.0447 & 24.7 & 19.7 & 32.6 & 0.512 & 1.15 & 5.90 & 5.94 & 6.09 & 7.17 & 0.0224  \\
    \bottomrule
    \end{tabular}%
  \label{tab:QM9}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 



==> [arxiv] Antibody/tabs/Task_specificity.tex <==
% Table generated by Excel2LaTeX from sheet 'Dataset'
\begin{table}[t]
  \centering\footnotesize
  \setlength{\tabcolsep}{3pt}
    \caption{Task antibody specificity. Summary of the statistical significance test of two antibody-specific features for different tasks in the \benchmark benchmark.}
    \begin{tabular}{cc|c|c}
    \toprule
    \multirow{2}{*}{\textbf{Task}} & \multicolumn{2}{c}{\textbf{Statistical significance
(p-value)}} & \multirow{2}{*}{\textbf{General Specificity}}  \\
    \cmidrule{2-3}  & \multicolumn{1}{c}{\textbf{Germline Usage}} & \multicolumn{1}{c}{\textbf{Mutations Numbers}} & \\
    \midrule
    Antigen Binding & Nan & Nan & Low \\
    Paratope Prediction & 0.296 & 0 & Medium \\
    %Disease Diagnosis & Disease Classification & Individual Profile & Q7 classification &  313  \\
    B cell classification  & 0 & 0 & High\\
    SARS antibody discovery  & 0 & 0 & High \\


    \bottomrule
    \end{tabular}%
  \label{tab:task_spec}%
\end{table}%





==> [arxiv] Antibody/tabs/Therapeutic.tex <==
% Table generated by Excel2LaTeX from sheet 'BCR'
\begin{table}[t]\footnotesize
  \centering\setlength{\tabcolsep}{2pt}
  \caption{Performance of PPLMs and PALMs on antibody tasks with increasing specificity. The reported results are the average of repetitive experiments with the standard derivation. \method w/o AGP indicates that we remove AGP objective from the pre-taining phase.}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{lrrr|rrr|r}
    \toprule
      & \multicolumn{3}{c}{\textbf{Antigen Binding (Low)}} & \multicolumn{3}{c}{\textbf{Paratope (Medium)}} & \textbf{ Cell (High)} \\
      %Specificity & \multicolumn{3}{c}{\textbf{Low}} & \multicolumn{3}{c}{\textbf{Medium}} & \multicolumn{1}{c}{\textbf{High}} 
    \cmidrule{2-8}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c|}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{ACC}} \\
    \midrule
    % Baseline* & 0.9100 & / & / & 0.8780$\pm$0.0040 & 0.6900$\pm$0.0060 & 0.5540$\pm$0.0060 \\
    % Ablang-H\citep{olsen2022ablang} & 0.9182$\pm$0.0007 & 0.8613$\pm$0.0029 & \textbf{0.7035}$\pm$0.0104 & 0.8780$\pm$0.0088 & 0.6741$\pm$0.0176 & 0.5457$\pm$0.0225 \\
    % Baseline* & 91.00 & / & / & 87.80$\pm$0.40 & 69.00$\pm$0.60 & 55.40$\pm$0.60 \\
    % Ablang-H\citep{olsen2022ablang} & 91.82$\pm$0.07 & 86.13$\pm$0.29 & \textbf{70.35}$\pm$1.04 & 87.80$\pm$0.88 & 67.41$\pm$1.76 & 54.57$\pm$2.25 \\
    % Baseline* & 0.910 & / & / & 0.878$\pm$0.004  & 0.690$\pm$0.006  & 0.554$\pm$0.006 & /  \\
    % \midrule
    non-pretrain & 0.858$\pm$0.014 & 0.584$\pm$0.330 & 0.432$\pm$0.183 & 0.845$\pm$0.014 & 0.605$\pm$0.033 & 0.463$\pm$0.037 & 0.554 $\pm$ 0.042 \\
    \midrule
    ESM-1~ & 0.917{\footnotesize$\pm$0.001} & 0.854{\footnotesize$\pm$0.002} & 0.689{\footnotesize$\pm$0.002} & 0.886{\footnotesize$\pm$0.009} & 0.669{\footnotesize$\pm$0.024} & 0.547{\footnotesize$\pm$0.026} & 0.503 {\footnotesize$\pm$ 0.031}\\
    % ESM-1 FT & 0.914{\footnotesize$\pm$0.001} & 0.858{\footnotesize$\pm$0.001} & 0.695{\footnotesize$\pm$0.003} & 0.883{\footnotesize$\pm$0.009} & 0.657{\footnotesize$\pm$0.031} & 0.534{\footnotesize$\pm$0.030} & ? \\
    %ESM-1b & \textbf{0.924$\pm$0.002} & 0.860$\pm$0.002 & \textbf{0.707$\pm$0.003} & 0.873$\pm$0.009 & 0.655$\pm$0.042 & 0.524$\pm$0.036 \\
    %ESM-1b FT & 0.916$\pm$0.003 & 0.844$\pm$0.003 & 0.686$\pm$0.004 & 0.869$\pm$0.010 & 0.660$\pm$0.021 & 0.527$\pm$0.015 \\
    MSA-1b & 0.921{\footnotesize$\pm$0.001} & 0.857$\pm$0.004 & 0.689$\pm$0.014 & 0.887$\pm$0.009 & 0.679$\pm$0.019 & 0.557$\pm$0.025 & 0.416 $\pm$ 0.050\\
    
    \midrule
    
    Ablang-H & 0.918$\pm$0.001 & 0.861$\pm$0.003 & \textbf{0.704$\pm$0.010} & 0.878$\pm$0.009 & 0.674$\pm$0.018 & 0.546$\pm$0.023 & 0.570 $\pm$ 0.010 \\
    Ablang-L & 0.917$\pm$0.002 & 0.856$\pm$0.001 & 0.682$\pm$0.001 & 0.882$\pm$0.010 & 0.680$\pm$0.018 & 0.553$\pm$0.023 & 0.546 $\pm$ 0.008 \\
    AntiBERT & 0.918$\pm$0.003 & 0.843$\pm$0.009 & 0.678$\pm$0.008 & 0.879$\pm$0.011 & 0.690$\pm$0.020 & 0.559$\pm$0.026 & 0.565 $\pm$ 0.028 \\
    \midrule
    \method & 0.922$\pm$0.004 & \textbf{0.862$\pm$0.004} & 0.699$\pm$0.010 & \textbf{0.887$\pm$0.008} & \textbf{0.698$\pm$0.017} & \textbf{0.575$\pm$0.024} & \textbf{0.581 $\pm$ 0.005}\\
    \method w/o \CGC & 0.920$\pm$0.003 & 0.855$\pm$0.000 & 0.697$\pm$0.008 & 0.883$\pm$0.011 & 0.676$\pm$0.021 & 0.552$\pm$0.027 & 0.559 $\pm$ 0.012 \\
    \method w/o \MPP & \textbf{0.923$\pm$0.001} & 0.855$\pm$0.002 & 0.687$\pm$0.005 & 0.883$\pm$0.011 & 0.691$\pm$0.022 & 0.566$\pm$0.030 & 0.563 $\pm$ 0.010\\
    \method w/o \CGC \& \MPP & 0.918$\pm$0.001 & 0.845$\pm$0.005 & 0.681$\pm$0.005 & 0.880$\pm$0.009 & 0.674$\pm$0.018 & 0.552$\pm$0.023 & 0.559 $\pm$ 0.009\\
    %\method-large & 0.921$\pm$0.004 & 0.854$\pm$0.004 & 0.677$\pm$0.010 & \textbf{0.887$\pm$0.007} & 0.685$\pm$0.015 & 0.561$\pm$0.020 \\
    
    \bottomrule
    \end{tabular}%
    }%
  \label{tab:specificity}%
\end{table}%



==> [arxiv] Antibody/tabs/case_study.tex <==
\begin{table}[b]\footnotesize
 \begin{minipage}[t]{0.55\linewidth}
 \vspace{10pt} % for top [t] alignment, bottom is [b]
    \centering
        \includegraphics[width=\linewidth]{figs/SARS_90.pdf}
        \caption{t90.}
        \label{fig:SARS_90}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.5\linewidth}
      \vspace{0pt}
            \centering
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\textwidth]{figs/health.germtype.pdf}
                \caption{Health germlines.}
                \label{fig:germ_health}
            \end{subfigure}
            % \hfill
            % \hspace{-7mm}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\textwidth]{figs/sars.germtype.pdf}
                \caption{Patient germlines.}
                \label{fig:germ_sars}
            \end{subfigure}
            % \vskip 0.1\baselineskip
            % \hspace{-4mm}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\textwidth]{figs/health.freq1000.pdf}
                \caption{Health distance.}
                % \vspace{-0.5\baselineskip}
                \label{fig:health_dist}
            \end{subfigure}
            % \hfill
            % \hspace{-8mm}
            \begin{subfigure}{0.45\textwidth}
               \includegraphics[width=\textwidth]{figs/sars.freq1000.pdf}
                \caption{Patient distance.}
                % \vspace{-0.5\baselineskip}
                \label{fig:sars_dist}
            \end{subfigure}
            \caption{UMAP Visualization. (a-b) for sequences with different germlines. One color indicates one germline with its descendant. (c-d) for evolutionary phylogeny distance. The shade of color indicate its distance from the ancestor germline.}
            \label{fig:germline}
  \end{minipage}
\end{table}

==> [arxiv] Antibody/tabs/cell.tex <==
% Table generated by Excel2LaTeX from sheet 'Cell'
\begin{table}[htbp]
  \centering
  \caption{Cell}
    \begin{tabular}{lr} 
    \toprule
    \textbf{Model} & \multicolumn{1}{c}{\textbf{ACC}} \\
    \midrule
    Ablang-H~\citep{olsen2022ablang} & 0.5695 \\
    Ablang-L~\citep{olsen2022ablang} & 0.5462 \\
    ESM-1b~\citep{rives2021biological} & 0.5030 \\
    \midrule
    Transformer & 0.5542 \\
    AntiBERT & 0.4646 \\
    \midrule
    \method & \textbf{0.5814} \\
    \method w/o \CGC & 0.5593 \\
    \method w/o \MPP & 0.5634 \\
    \method w/o \CGC \& \MPP & 0.5591 \\
    \bottomrule
    \end{tabular}%
  \label{tab:cell}%
\end{table}%


==> [arxiv] Antibody/tabs/cell_analysis.tex <==
% Table generated by Excel2LaTeX from sheet 'Cell'
% \begin{table}[htbp]
%   \centering\small
%   \setlength{\tabcolsep}{1pt}
%   \caption{Cell Analysis}
%     \begin{tabular}{lcccccc}
%     \toprule
%       & \multicolumn{1}{l}{\textbf{Immature B}} & \multicolumn{1}{l}{\textbf{Memory IgD-}} & \multicolumn{1}{l}{\textbf{Memory IgD+}} & \multicolumn{1}{l}{\textbf{Plasmacytes PC}} & \multicolumn{1}{l}{\textbf{Transitional B}} & \multicolumn{1}{l}{\textbf{Mature B}} \\
%     \midrule
%     \textbf{Immature B} & 89.59 & 1.63 & 1.50 & 1.63 & 4.15 & 1.50 \\
%     \textbf{Memory IgD-} & 2.63 & 50.18 & 9.58 & 15.93 & 7.90 & 13.77 \\
%     \textbf{Memory IgD+} & 1.83 & 5.12 & 44.62 & 17.34 & 12.22 & 18.87 \\
%     \textbf{Plasmacytes PC} & 1.81 & 4.95 & 12.57 & 59.85 & 8.26 & 12.57 \\
%     \textbf{Transitional B} & 3.70 & 4.85 & 16.02 & 18.03 & 40.60 & 16.80 \\
%     \textbf{Mature B} & 2.14 & 5.26 & 15.59 & 18.22 & 13.33 & 45.48 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:cell_analysis}%
% \end{table}%


\begin{table}[b]\footnotesize
 \begin{minipage}[t]{0.45\linewidth}
 \vspace{0pt} % for top [t] alignment, bottom is [b]
    \centering
    \caption{B cell classification (Q6). \textbf{ACC} is the prediction accuracy. The details are in Section \ref{sec:task} and \ref{sec:method}. The best result is bolded.}
   \label{tab:cell}%
   \footnotesize\setlength{\tabcolsep}{3pt}
    \begin{tabular}{lr}
        \toprule
        \textbf{Model} & \multicolumn{1}{c}{\textbf{ACC}} \\
        \midrule
        No Pretrain & 0.554 $\pm$ 0.042\\
        \midrule
        ESM-1~\citep{rives2021biological} & 0.503 $\pm$ 0.031 \\
        ESM-1 FT \\
        MSA-1b~\citep{rao2021msa} & 0.416 $\pm$ 0.050 \\
        \midrule
        Ablang-H~\citep{olsen2022ablang} & 0.570 $\pm$ 0.010 \\
        Ablang-L~\citep{olsen2022ablang} & 0.546 $\pm$ 0.008 \\
        AntiBERT & 0.565 $\pm$ 0.028\\
        \midrule
        %Transformer & 0.554 $\pm$ 0.042\\
        \method & \textbf{0.581 $\pm$ 0.005} \\
        \method w/o \CGC & 0.559 $\pm$ 0.012 \\
        \method w/o \MPP & 0.563 $\pm$ 0.010 \\
        \method w/o \CGC \& \MPP & 0.559 $\pm$ 0.009\\
        \bottomrule
    \end{tabular}%
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.5\linewidth}
  \vspace{0pt}
      \centering
    %   \begin{figure}
        \includegraphics[width=\textwidth]{figs/cell.pdf}
        \caption{Category prediction. For each $p_{ij}$ in $i-$th row and $j$-th column, it means the frequency for the model to predict a sequence in $i$ category to $j$ category. The number is normalized by row.}
        \label{fig:cell_analysis}
    % \end{figure}
  \end{minipage}
\end{table}


==> [arxiv] Antibody/tabs/cellds.tex <==
% Table generated by Excel2LaTeX from sheet 'Cell'
\begin{table}[htbp]
  \centering
  \caption{The statistics of B cell classification.}
    \begin{tabular}{lc}
    \toprule
    \textbf{Type} & \multicolumn{1}{c}{\textbf{Size}} \\
    \midrule
    Immature b cell & 14,145  \\
    Transitional b cell &  13,197  \\
    Mature b cell &  16,139  \\
    Plasmacytes PC &   22,236  \\
    Memory IgD- &   8,437  \\
    Memory IgD+ &   13,940  \\
    \bottomrule
    \end{tabular}%
  \label{tab:cellds}%
\end{table}%


==> [arxiv] Antibody/tabs/discovery.tex <==
% Table generated by Excel2LaTeX from sheet 'Cell'
% \begin{table}[htbp]
%   \centering\small
%   \setlength{\tabcolsep}{1pt}
%   \caption{Cell Analysis}
%     \begin{tabular}{lcccccc}
%     \toprule
%       & \multicolumn{1}{l}{\textbf{Immature B}} & \multicolumn{1}{l}{\textbf{Memory IgD-}} & \multicolumn{1}{l}{\textbf{Memory IgD+}} & \multicolumn{1}{l}{\textbf{Plasmacytes PC}} & \multicolumn{1}{l}{\textbf{Transitional B}} & \multicolumn{1}{l}{\textbf{Mature B}} \\
%     \midrule
%     \textbf{Immature B} & 89.59 & 1.63 & 1.50 & 1.63 & 4.15 & 1.50 \\
%     \textbf{Memory IgD-} & 2.63 & 50.18 & 9.58 & 15.93 & 7.90 & 13.77 \\
%     \textbf{Memory IgD+} & 1.83 & 5.12 & 44.62 & 17.34 & 12.22 & 18.87 \\
%     \textbf{Plasmacytes PC} & 1.81 & 4.95 & 12.57 & 59.85 & 8.26 & 12.57 \\
%     \textbf{Transitional B} & 3.70 & 4.85 & 16.02 & 18.03 & 40.60 & 16.80 \\
%     \textbf{Mature B} & 2.14 & 5.26 & 15.59 & 18.22 & 13.33 & 45.48 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:cell_analysis}%
% \end{table}%


\begin{table}[htbp]\footnotesize
\setlength{\tabcolsep}{1pt}
 \begin{minipage}[t]{0.7\linewidth}
 % \vspace{0pt} % for top [t] alignment, bottom is [b]
    \caption{The CDR3-H3 region of high-ranked sequences to bind to SARS. We show the CDR3 fragment of the heavy chain in the antibody sequences. `Identity' is the similarity between the predicted binder and the true binder. The epitope of the true binders is shown. The origin of the majority of the true binder sequences is B cells from patients. The different amino acids between the predicted binder and the existing binder are highlighted in red}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{rlllcc}
    \toprule
    % \vspace{10pt}
    \textbf{No}  & \textbf{Predicted Binder} & \textbf{Existing Binder} & \textbf{Epitope} & \textbf{Identity} \\
    \midrule
    1 & AREGIVGATTGFDY & AREGIVGATTGFDY & spike & 1.000 \\
    2 & ARDLGGYFDY & ARDLGGYFDY & RBD & 1.000 \\
    3 & AKDQDD\textcolor{red}{A}YYYYYYMDV & AKDQDD\textcolor{red}{G}YYYYYYMDV & NTD & 0.938 \\
    4 & ASYYYDSSGY\textcolor{red}{H}YGMDV & ASYYYDSSGY\textcolor{red}{Y}YGMDV & RBD & 0.938 \\
    5 & ARRG\textcolor{red}{L}GLYYYGMDV & ARRG\textcolor{red}{D}GLYYYGMDV & S2 & 0.929 \\
    6 & ARA\textcolor{red}{F}RGSYYYGMDV & ARA\textcolor{red}{T}RGSYYYGMDV & S2 & 0.929 \\
    7 & ARLSGSSW\textcolor{red}{Y}FDY & ARLSGSSW\textcolor{red}{D}FDY & spike & 0.917 \\
    8 & AR\textcolor{red}{L}GSSSWYFDY & AR\textcolor{red}{V}GSSSWYFDY & spike & 0.917 \\
    9 & ARGWLRGYFDL & AR\textcolor{red}{R}GWLRGYFDL & RBD & 0.909 \\
    10 & ARDWGE\textcolor{red}{L}YFDY & ARDWGE\textcolor{red}{Y}YFDY & RBD & 0.909 \\
    11 & ARDLGG\textcolor{red}{V}FDY & ARDLGG\textcolor{red}{Y}FDY & RBD & 0.900 \\
    \bottomrule
    \end{tabular}%
    }%
    \label{tab:11binder}%
    \end{minipage}
    \hfill
    % \vspace{-10pt}
    \begin{minipage}[t]{0.25\linewidth}
      \centering
        \caption{3D structure of the true SARS-CoV-2 binding antibody No.3. G2A highlights the single atom difference in No.3, indicating the predicted binder is highly likely to bind the virus.}
         \vspace{-25pt}
         \includegraphics[width=\linewidth]{figs/3D_1.pdf}
         \label{fig:3d_binder}
  \end{minipage}
\end{table}
\vspace{-25pt}


 


==> [arxiv] Antibody/tabs/disease.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease'
\begin{table}[t]
  \centering\footnotesize
  \setlength{\tabcolsep}{2pt}
  \caption{Disease Diagnosis. The definition of notation \textbf{AUC}, \textbf{F1}, \textbf{MCC} can be found in Section \ref{sec:benchmark}. The full table with more diseases and standard deviations can be found in Appendix.}
  
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[1]{*}{\textbf{Individual-level}}} & \multicolumn{3}{c}{\textbf{SARS}} & \multicolumn{3}{c}{\textbf{HIV}} & \multicolumn{3}{c}{\textbf{Ebola}} \\
    \cmidrule{2-10}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    Ablang-H & 0.988 & 0.968 & 0.920 & 0.960 & 0.788 & 0.744 & 0.944 & 0.767 & 0.750 \\
    Ablang-L & \textbf{0.990} & 0.938 & 0.843 & 0.931 & 0.798 & 0.742 & 0.961 & 0.731 & 0.703 \\
    ESM-1 & 0.979 & 0.933 & 0.824 & 0.967 & 0.883 & 0.849 & \textbf{1.000} & 0.933 & 0.934 \\
    MSA-1b & 0.989 & 0.954 & 0.887 & 0.962 & 0.833 & 0.789 & \textbf{1.000} & 0.933 & 0.934 \\
    \midrule
    Transformer & 0.975 & 0.962 & 0.902 & 0.920 & 0.815 & 0.776 & 0.994 & 0.933 & 0.934 \\
    AntiBERT & 0.983 & 0.976 & 0.938 & 0.969 & 0.878 & 0.850 & 0.978 & 0.933 & 0.934 \\
    \midrule
    \method & 0.977 & \textbf{0.983} & \textbf{0.955} & \textbf{0.978} & 0.914 & 0.884 & \textbf{1.000} & \textbf{0.947} & \textbf{0.944} \\
    \method w/o \CGC & 0.983 & 0.973 & 0.929 & \textbf{0.978} & 0.903 & 0.869 & \textbf{1.000} & 0.933 & 0.934 \\
    \method w/o \MPP & 0.987 & 0.969 & 0.921 & 0.976 & 0.906 & 0.880 & \textbf{1.000} & 0.933 & 0.934 \\
    \method w/o \CGC \& \MPP & 0.986 & 0.969 & 0.920 & 0.973 & \textbf{0.919} & \textbf{0.896} & 0.994 & 0.933 & 0.934 \\
    \bottomrule
    \end{tabular}%
  \label{tab:disease}%
\end{table}%


==> [arxiv] Antibody/tabs/disease_q7.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease (2)'
\begin{table}[htbp]\small
  \centering\setlength{\tabcolsep}{1.0pt}
  \caption{The Q7 disease classification task. `ACC' is the accuracy rate.}
  \label{tab:disease_q7}%
    \begin{tabular}{ll}
    \toprule
    \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{ACC}} \\
    \midrule
    No pretrain & 0.754$\pm$0.023 \\
    \midrule
    ESM-1 & 0.747$\pm$0.016 \\
    ESM-1 FT & \textbf{0.762$\pm$0.024} \\
    %ESM-1b & 0.692$\pm$0.036 \\
    %ESM-1b FT & 0.690$\pm$0.029 \\
    MSA-1b & 0.746$\pm$0.019 \\
    \midrule
    Ablang-H & 0.704$\pm$0.033 \\
    Ablang-L & 0.702$\pm$0.040 \\
    AntiBERT & 0.750$\pm$0.016 \\
    \midrule
    \method & \textbf{0.756$\pm$0.020} \\
    \method w/o \CGC & 0.754$\pm$0.020 \\
    \method w/o \MPP & 0.755$\pm$0.020 \\
    \method w/o \CGC \& \MPP & 0.756$\pm$0.021 \\
    %\method-large & 0.743$\pm$0.020 \\
    \bottomrule
    \end{tabular}%
\end{table}%



==> [arxiv] Antibody/tabs/disease_seq.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease'
\begin{table}[htbp]
  \centering\footnotesize
  \setlength{\tabcolsep}{3pt}
  \caption{Sequence-level predictor for disease diagnosis. The definition of notation are the same as the Table 4 in main body.}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[1]{*}{\textbf{Sequence-level}}} & \multicolumn{3}{c}{\textbf{SARS}} & \multicolumn{3}{c}{\textbf{HIV}} & \multicolumn{3}{c}{\textbf{Ebola}} \\
    \cmidrule{2-10}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    Ablang-H & 0.9151 & \textbf{0.8166} & \textbf{0.6679} & 0.8948 & 0.6842 & 0.6036 & 0.9514 & 0.7003 & 0.6908 \\
    Ablang-L & 0.8929 & 0.8012 & 0.6372 & 0.8813 & 0.6682 & 0.5842 & 0.9450 & 0.7185 & 0.7096 \\
    ESM-1b & 0.9032 & 0.7992 & 0.6476 & 0.9268 & 0.7386 & \textbf{0.7008} & \textbf{0.9704} & 0.8447 & 0.8357 \\
    \midrule
    Transformer & 0.8939 & 0.8007 & 0.6367 & 0.8928 & 0.6224 & 0.5625 & 0.9665 & 0.7960 & 0.7869 \\
    AntiBERT & \textbf{0.9155} & 0.8101 & 0.6606 & 0.9213 & 0.7422 & 0.6893 & 0.9591 & 0.8043 & 0.7952 \\
    \midrule
    \method & 0.9043 & 0.8081 & 0.6434 & 0.9297 & 0.7438 & 0.6768 & 0.9689 & \textbf{0.8484} & \textbf{0.8407} \\
    \method w/o \CGC & 0.9040 & 0.8083 & 0.6442 & \textbf{0.9326} & 0.7473 & 0.6786 & 0.9671 & 0.8426 & 0.8346 \\
    \method w/o \MPP & 0.9011 & 0.8081 & 0.6484 & 0.9319 & 0.7485 & 0.6822 & 0.9694 & 0.8404 & 0.8284 \\
    \method w/o \CGC \& \MPP & 0.9010 & 0.8074 & 0.6446 & 0.9303 & \textbf{0.7492} & 0.6784 & 0.9699 & 0.8208 & 0.8113 \\
    \bottomrule
    \end{tabular}%
  \label{tab:disease_seq}%
\end{table}%




==> [arxiv] Antibody/tabs/hit_rate.tex <==
% Table generated by Excel2LaTeX from sheet 

\begin{table}[htbp]
  \centering
  \caption{SARS-CoV-2 antibody hit rate with different probability thresholds. `Total' is the total number of sequences whose probabilities are higher than the threshold. `Hit' is the number of sequences that meet the similarity requirements with existing binders.  }
  \label{tab:hit_rate}%
    \begin{tabular}{ccccc}
    \toprule
    \textbf{Threshold}  & \textbf{Total} & \textbf{Hit} & \textbf{Hit rate (\%)} \\
    \midrule
        0.5 & 13253 & 66 & 0.498 \\
        0.7 & 10227 & 54 & 0.528 \\
        0.8 & 9338 & 49 & 0.525 \\
        0.9 & 8178 & 47 & 0.562 \\
    \bottomrule
    \end{tabular}%
\end{table}%


==> [arxiv] Antibody/tabs/newbinder.tex <==
% Table generated by Excel2LaTeX from sheet 'New binder'

\begin{table}[htbp]\footnotesize
   \setlength{\tabcolsep}{2.8pt}
  \centering
  \caption{The CDR3-H3 region of high-ranked sequences to bind to SARS. We show the CDR3 fragment of the heavy chain in the antibody sequences. `Identity' is the similarity between the predicted binder and the true binder. The epitope of the true binders are shown. The difference amino acids between predicted binder and true binder are highlighted in red}
  %Binder No.16 comes from semi-synthetic library and binind No. 32 and No. 34 from Phage display. 'unk' stands for unknown.}
    \begin{tabular}{rlllcc}
    \toprule
    \textbf{No}  & \textbf{Predicted Binder} & \textbf{Existing Binder} & \textbf{Epitope} & \textbf{Identity $\uparrow$ } \\
    \midrule
    1 & AREGIVGATTGFDY & AREGIVGATTGFDY & spike & 1.000 \\
    2 & ARDLGGYFDY & ARDLGGYFDY & RBD & 1.000 \\
    3 & AKDQDD\textcolor{red}{A}YYYYYYMDV & AKDQDD\textcolor{red}{G}YYYYYYMDV & NTD & 0.938 \\
    4 & ASYYYDSSGY\textcolor{red}{H}YGMDV & ASYYYDSSGY\textcolor{red}{Y}YGMDV & RBD & 0.938 \\
    5 & ARRG\textcolor{red}{L}GLYYYGMDV & ARRG\textcolor{red}{D}GLYYYGMDV & S2 & 0.929 \\
    6 & ARA\textcolor{red}{F}RGSYYYGMDV & ARA\textcolor{red}{T}RGSYYYGMDV & S2 & 0.929 \\
    7 & ARLSGSSW\textcolor{red}{Y}FDY & ARLSGSSW\textcolor{red}{D}FDY & spike & 0.917 \\
    8 & AR\textcolor{red}{L}GSSSWYFDY & AR\textcolor{red}{V}GSSSWYFDY & spike & 0.917 \\
    9 & AR\textcolor{red}{-}GWLRGYFDL & AR\textcolor{red}{R}GWLRGYFDL & RBD & 0.909 \\
    10 & ARDWGE\textcolor{red}{L}YFDY & ARDWGE\textcolor{red}{Y}YFDY & RBD & 0.909 \\
    11 & ARDLGG\textcolor{red}{V}FDY & ARDLGG\textcolor{red}{Y}FDY & RBD & 0.900 \\
    %12 & ARGDSSGWYTGDVFDI & ARVDSSGWYTGDVFDV & RBD & 0.875 \\
    %13 & ARGDSDSSGYYYYFDY & ARGDSSGYYYYFDY & RBD & 0.871 \\
    %14 & ARHRAAGGNYYYGMDV & ARAAGGNYYYGMDV & RBD & 0.875 \\
    %15 & AAPYCSGGSCTDAFDI & AAPYCSGGSCFDAFDM & RBD & 0.875 \\
    %16 & AKDRYYYDSSGYYEYYYYYGMDV & ARDRYYYDSSGYYYDYYYGMDV & RBD & 0.870 \\
    %17 & AKGDTAMAPYNWFDP & AKADTAMAWYNWFDP & NTD & 0.867 \\
    %18 & ARAPGSSYSSGWYDYYYGMDV & ARAPGASYSSGWYHYYYYMDV & RBD & 0.857 \\
    %19 & ATGVAVAGTPRYYYYYYGMDV & ATGVAVAGTPSSYYYYYYMDV & spike & 0.857 \\
    %20 & AVNSNYYYYYGMDV & ARYSNYYYYYGMDV & NTD & 0.857 \\
    %21 & ASYQNYYYYYGMDV & ARYSNYYYYYGMDV & NTD & 0.857 \\
    %22 & ARPRSGSYRDYFDY & ARPRSGSYYAYFDY & spike & 0.857 \\
    %23 & ARARGGSYLYGMDV & ARARGGNYYYGMDV & S2 & 0.857 \\
    %24 & ARSYSGSYYSRFDY & ARTYSGSYYSYFDY & S2 & 0.857 \\
    %25 & ARPFGGSYYSGFDY & ARPHGGSYYSYFDY & S2 & 0.857 \\
    %26 & ASGIAATYYYYMDV & ARGPAATYYYYMDV & spike & 0.857 \\
    %27 & AKDRAGNYYYGMDV & ARDRSGNYYYGMDV & spike & 0.857 \\
    %28 & ARDGIVGATTGLDY & ARDGMVGATTGIDY & S2 & 0.857 \\
    %29 & ARNRGGSYLGAFDI & ARARGGSYSGAFDI & unk & 0.857 \\
    %30 & ARGNSSGWSYYFDY & ARGDSNGWSYYFDY & spike & 0.857 \\
    %31 & ARLGSGSYSNWFDP & ARSGSGSYFNWFDP & S2 & 0.857 \\
    %32 & ARAMGGSYYGGMDV & ARARGGSYYYGMDV & S2 & 0.857 \\
    %33 & ARPTSGGYYYGMDV & ARAYSGGYYYGMDV & S2 & 0.857 \\
    %34 & ATSAVAGTPNWFDP & ATSRVAGTPNWFHP & NTD & 0.857 \\
    %35 & AREDYYDSSGAFDI & AREDYYDSSGSFDH & RBD & 0.857 \\
    %36 & ARRGHGLYYHGMDV & ARRGDGLYYYGMDV & unk & 0.857 \\
    %37 & ARDRGYCSSTSCYYYYGMDV & ARDDIGYCSSTSCSYYYYGMDV & spike & 0.850 \\
    \bottomrule
    \end{tabular}%
  \label{tab:newbinder}%
\end{table}%





==> [arxiv] Antibody/tabs/newbinder2.tex <==
% Table generated by Excel2LaTeX from sheet 'sars.highprob08.sorted.uniq'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{rllrr}
      \textbf{No}  & \textbf{CDR-H3 of predicted binder} & \textbf{CDR-H3 of  true binder} & \textbf{Identity} & \textbf{Score} \\
    1 & AREGIVGATTGFDY & AREGIVGATTGFDY & 1.0000 & 1.0000 \\
    2 & ARDLGGYFDY & ARDLGGYFDY & 1.0000 & 1.0000 \\
    3 & ARDLGGYFDY &  ARDLGGYFDY & 0.9312 & 1.0000 \\
    4 & AKDQDDAYYYYYYMDV & AKDQDDGYYYYYYMDV & 0.9645 & 0.9375 \\
    5 & ASYYYDSSGYHYGMDV & ASYYYDSSGYYYGMDV & 0.8858 & 0.9375 \\
    6 & ARRGLGLYYYGMDV & ARRGDGLYYYGMDV & 1.0000 & 0.9286 \\
    7 & ARAFRGSYYYGMDV & ARATRGSYYYGMDV & 1.0000 & 0.9286 \\
    8 & ARLSGSSWYFDY & ARLSGSSWDFDY & 0.9765 & 0.9167 \\
    9 & ARLGSSSWYFDY & ARVGSSSWYFDY & 0.9344 & 0.9167 \\
    10 & ARGWLRGYFDL & ARRGWLRGYFDL & 0.9996 & 0.9091 \\
    11 & ARDWGELYFDY & ARDWGEYYFDY & 0.8164 & 0.9091 \\
    12 & ARGDSSGWYTGDVFDI & ARVDSSGWYTGDVFDV & 1.0000 & 0.8750 \\
    13 & ARGDSDSSGYYYYFDY & ARGDSSGYYYYFDY & 1.0000 & 0.8750 \\
    14 & ARHRAAGGNYYYGMDV & ARAAGGNYYYGMDV & 0.9218 & 0.8750 \\
    15 & AAPYCSGGSCTDAFDI & AAPYCSGGSCFDAFDM & 0.8742 & 0.8750 \\
    16 & AKDRYYYDSSGYYEYYYYYGMDV & ARDRYYYDSSGYYYDYYYGMDV & 0.9968 & 0.8696 \\
    17 & AKGDTAMAPYNWFDP & AKADTAMAWYNWFDP & 1.0000 & 0.8667 \\
    18 & ARAPGSSYSSGWYDYYYGMDV & ARAPGASYSSGWYHYYYYMDV & 1.0000 & 0.8571 \\
    19 & ATGVAVAGTPRYYYYYYGMDV & ATGVAVAGTPSSYYYYYYMDV & 1.0000 & 0.8571 \\
    20 & AVNSNYYYYYGMDV & ARYSNYYYYYGMDV & 0.9999 & 0.8571 \\
    21 & ASYQNYYYYYGMDV & ARYSNYYYYYGMDV & 0.9981 & 0.8571 \\
    22 & ARPRSGSYRDYFDY & ARPRSGSYYAYFDY & 0.9925 & 0.8571 \\
    23 & ARARGGSYLYGMDV & ARARGGNYYYGMDV & 0.9922 & 0.8571 \\
    24 & ARSYSGSYYSRFDY & ARTYSGSYYSYFDY & 0.9819 & 0.8571 \\
    25 & ARPFGGSYYSGFDY & ARPHGGSYYSYFDY & 0.9738 & 0.8571 \\
    26 & ASGIAATYYYYMDV & ARGPAATYYYYMDV & 0.9677 & 0.8571 \\
    27 & AKDRAGNYYYGMDV & ARDRSGNYYYGMDV & 0.9365 & 0.8571 \\
    28 & ARDGIVGATTGLDY & ARDGMVGATTGIDY & 0.9365 & 0.8571 \\
    29 & ARNRGGSYLGAFDI & ARARGGSYSGAFDI & 0.9101 & 0.8571 \\
    30 & ARGNSSGWSYYFDY & ARGDSNGWSYYFDY & 0.9096 & 0.8571 \\
    31 & ARLGSGSYSNWFDP & ARSGSGSYFNWFDP & 0.8885 & 0.8571 \\
    32 & ARAMGGSYYGGMDV & ARARGGSYYYGMDV & 0.8786 & 0.8571 \\
    33 & ARPTSGGYYYGMDV & ARAYSGGYYYGMDV & 0.8779 & 0.8571 \\
    34 & ARDRGYCSSTSCYYYYGMDV & ARDDIGYCSSTSCSYYYYGMDV & 0.9499 & 0.8500 \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> [arxiv] Antibody/tabs/patient_level_full.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease'
\begin{table}[htbp]
  \centering\footnotesize
  \setlength{\tabcolsep}{1.5pt}
  \caption{Individual-level predictor for disease diagnosis. }
  \label{tab:patient_full_all}%
    \begin{tabular}{lrrr|rrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[3]{*}{\textbf{Pateint-level}}} & \multicolumn{3}{c}{\textbf{SARS}} & \multicolumn{3}{c}{\textbf{HIV}} \\
    \cmidrule{2-7}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    No pretrain & 0.975$\pm$0.033 & 0.962$\pm$0.024 & 0.902$\pm$0.062 & 0.920$\pm$0.092 & 0.815$\pm$0.117 & 0.776$\pm$0.122 \\
    \midrule
    ESM-1 & 0.979$\pm$0.017 & 0.933$\pm$0.032 & 0.824$\pm$0.090 & 0.967$\pm$0.056 & 0.883$\pm$0.107 & 0.849$\pm$0.135 \\
    MSA-1b & 0.989$\pm$0.012 & 0.954$\pm$0.033 & 0.887$\pm$0.078 & 0.962$\pm$0.039 & 0.833$\pm$0.068 & 0.789$\pm$0.072 \\
    \midrule
    Ablang-H & 0.988$\pm$0.013 & 0.968$\pm$0.024 & 0.920$\pm$0.063 & 0.960$\pm$0.040 & 0.788$\pm$0.134 & 0.744$\pm$0.137 \\
    Ablang-L & \textbf{0.990$\pm$0.015} & 0.938$\pm$0.039 & 0.843$\pm$0.091 & 0.931$\pm$0.069 & 0.798$\pm$0.131 & 0.742$\pm$0.170 \\
    AntiBERT & 0.983$\pm$0.017 & 0.976$\pm$0.022 & 0.938$\pm$0.056 & 0.969$\pm$0.053 & 0.878$\pm$0.112 & 0.850$\pm$0.134 \\
    \midrule
    \method & 0.977$\pm$0.028 & \textbf{0.983$\pm$0.017} & \textbf{0.955$\pm$0.045} & \textbf{0.978$\pm$0.054} & 0.914$\pm$0.081 & 0.884$\pm$0.106 \\
    \method w/o \CGC & 0.983$\pm$0.019 & 0.973$\pm$0.025 & 0.929$\pm$0.066 & \textbf{0.978$\pm$0.054} & 0.903$\pm$0.076 & 0.869$\pm$0.099 \\
    \method w/o \MPP & 0.987$\pm$0.015 & 0.969$\pm$0.024 & 0.921$\pm$0.061 & 0.976$\pm$0.053 & 0.906$\pm$0.092 & 0.880$\pm$0.112 \\
    \method w/o \MPP \& \CGC & 0.986$\pm$0.014 & 0.969$\pm$0.023 & 0.920$\pm$0.061 & 0.973$\pm$0.052 & \textbf{0.919$\pm$0.096} & \textbf{0.896$\pm$0.117} \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{} & \multicolumn{3}{c}{\textbf{Ebola}} & \multicolumn{3}{c}{\textbf{Allergy}} \\
    \cmidrule{2-7}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    No Pretrain & 0.994$\pm$0.017 & 0.933$\pm$0.133 & 0.934$\pm$0.132 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \midrule
    ESM-1 & 1.000$\pm$0.000 & 0.933$\pm$0.133 & 0.934$\pm$0.132 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    MSA-1b & 1.000$\pm$0.000 & 0.933$\pm$0.133 & 0.934$\pm$0.132 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \midrule
    Ablang-H & 0.944$\pm$0.167 & 0.767$\pm$0.213 & 0.750$\pm$0.254 & 1.000$\pm$0.000 & 0.960$\pm$0.080 & 0.916$\pm$0.169 \\
    Ablang-L & 0.961$\pm$0.100 & 0.731$\pm$0.205 & 0.703$\pm$0.277 & 1.000$\pm$0.000 & 0.960$\pm$0.080 & 0.916$\pm$0.169 \\
    AntiBERT & 0.978$\pm$0.067 & 0.933$\pm$0.133 & 0.934$\pm$0.132 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \midrule
    \method & 1.000$\pm$0.000 & \textbf{0.947$\pm$0.111} & \textbf{0.944$\pm$0.114} & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \method w/o \CGC & 1.000$\pm$0.000 & 0.933$\pm$0.133 & 0.934$\pm$0.132 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \method w/o \MPP & 1.000$\pm$0.000 & 0.933$\pm$0.133 & 0.934$\pm$0.132 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \method w/o \MPP \& \CGC & 0.994$\pm$0.017 & 0.933$\pm$0.133 & 0.934$\pm$0.132 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \midrule
    \midrule
    \multirow{2}[3]{*}{} & \multicolumn{3}{c}{\textbf{SLE}} & \multicolumn{3}{c}{\textbf{MS}} \\
    \cmidrule{2-7}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    No Pretrain & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.700$\pm$0.200 & 0.900$\pm$0.137 & 0.893$\pm$0.400 \\
    \midrule
    ESM-1 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.900$\pm$0.200 & 0.933$\pm$0.133 & 0.900$\pm$0.200 \\
    MSA-1b & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.700$\pm$0.400 & 0.893$\pm$0.137 & 0.700$\pm$0.400 \\
    \midrule
    Ablang-H & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.800$\pm$0.245 & 0.893$\pm$0.137 & 0.700$\pm$0.400 \\
    Ablang-L & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.960$\pm$0.080 & 0.800$\pm$0.400 \\
    AntiBERT & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 \\
    \midrule
    \method & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.867$\pm$0.163 & 0.800$\pm$0.245 \\
    \method w/o \CGC & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.867$\pm$0.163 & 0.800$\pm$0.245 \\
    \method w/o \MPP & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.827$\pm$0.150 & 0.600$\pm$0.374 \\
    \method w/o \MPP \& \CGC & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 1.000$\pm$0.000 & 0.827$\pm$0.150 & 0.800$\pm$0.374 \\
    \bottomrule
    \label{individual_level}
    \end{tabular}%
\end{table}%


==> [arxiv] Antibody/tabs/pretrained.tex <==
% % Table generated by Excel2LaTeX from sheet 'Pretrained'
% \begin{table}[htbp]
%   \centering
%   \caption{Pretrained Model}
%     \begin{tabular}{lrr}
%     \toprule
%     \textbf{Model} & \multicolumn{1}{c}{\textbf{Loss}} & \multicolumn{1}{c}{\textbf{Step}} \\
%     \midrule
%     % BERT & 0.437 & 568000 \\
%     % BERT + contrastive & 0.558 & 19000 \\
%     % BERT + mutation & 1.744 & 134000 \\
%     EALM w/o \MPP \& \CGC  & 0.143 & 108000 \\
%     EALM w/o \CGC & 1.744 & 134000 \\
%     EALM w/o \MPP & 0.001 & 18000 \\    
%     EALM  & 1.856 & 54000 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:pretrain}%
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Pretrained'
\begin{table}[htbp]\footnotesize
  \centering
  \caption{The pretraining details for different models. The `Germline' is the prediction accuracy of \CGC, and the `Position' and `Mutation' are the accuracy of mutation positions and the mutated residues respectively.}
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Size}}& \multicolumn{1}{c}{\textbf{Loss}} & \multicolumn{1}{c}{\textbf{Step}} & \textbf{Germline} & \textbf{Position} & \textbf{Mutation} \\
    \midrule
    AntiBERT & 85M & 0.437 & 568000 & / & / & 0.031 \\
    AntiBERT w \CGC & 85M& 0.558 & 587000 & 0.330 & / & / \\
    AntiBERT w \MPP & 85M& 1.744 & 622000 & / & 0.965 & 0.410 \\
    \midrule
    ESM-1 FT & 85M& 0.2636 & 136000 & / & / & / \\
    ESM-1b FT & 650M & 0.2704 & 278000 & / & / & / \\
    \midrule
    \midrule
    \method w/o \CGC \& \MPP & 85M& 0.143 & 108000 & / & / & / \\
    \method w/o \CGC & 85M& 1.744 & 134000 & / & 1.000 & 0.442 \\
    \method w/o \MPP & 85M& 0.001 & 126000 & 1.000 & / & / \\
    \method  & 85M & 1.856 & 252500 & 0.996 & 1.000 & 0.443 \\
    \midrule
    \method-large w/o \CGC \& \MPP & 650M & 0.149 & 193000 & / & / & / \\
    \method-large w/o \CGC & 650M & 1.753 & 267000 & / & 1.000 & 0.438 \\
    \method-large w/o \MPP & 650M & 0.001 & 200000 & 1.000 & / & / \\
    \method-large & 650M & 1.773 & 384000 & 0.996 & 1.000 & 0.431 \\
    \bottomrule
    \end{tabular}%
  \label{tab:pretrain}%
\end{table}%



==> [arxiv] Antibody/tabs/sequence_level_full.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease'
\begin{table}[htbp]
  \centering\footnotesize
  \setlength{\tabcolsep}{1.5pt}
  \caption{Sequence-level predictor for disease diagnosis.}
  \label{tab:sequence_full_all}%
    \begin{tabular}{lrrr|rrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[3]{*}{\textbf{Sequence-level}}} & \multicolumn{3}{c}{\textbf{SARS}} & \multicolumn{3}{c}{\textbf{HIV}} \\
    \cmidrule{2-4} \cmidrule{5-7}
    & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} &  \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    No Pretrain & 0.894$\pm$0.029 & 0.801$\pm$0.045 & 0.637$\pm$0.078 & 0.893$\pm$0.081 & 0.622$\pm$0.223 & 0.563$\pm$0.209 \\
    \midrule
    ESM-1 & 0.903$\pm$0.061 & 0.799$\pm$0.032 & 0.648$\pm$0.093 & 0.927$\pm$0.039 & 0.739$\pm$0.082 & \textbf{0.701$\pm$0.080} \\
    MSA-1b & 0.914$\pm$0.025 & 0.810$\pm$0.050 & \textbf{0.671$\pm$0.080} & 0.903$\pm$0.064 & 0.680$\pm$0.103 & 0.617$\pm$0.102 \\
    \midrule
    Ablang-H & 0.915$\pm$0.027 & \textbf{0.817$\pm$0.038} & 0.668$\pm$0.068 & 0.895$\pm$0.058 & 0.684$\pm$0.087 & 0.604$\pm$0.108 \\
    Ablang-L & 0.893$\pm$0.035 & 0.801$\pm$0.054 & 0.637$\pm$0.099 & 0.881$\pm$0.072 & 0.668$\pm$0.111 & 0.584$\pm$0.131 \\
    AntiBERT & \textbf{0.916$\pm$0.026} & 0.810$\pm$0.033 & 0.661$\pm$0.060 & 0.921$\pm$0.046 & 0.742$\pm$0.088 & 0.689$\pm$0.101 \\
    \midrule
    \method & 0.904$\pm$0.027 & 0.808$\pm$0.035 & 0.643$\pm$0.069 & 0.930$\pm$0.044 & 0.744$\pm$0.079 & 0.677$\pm$0.105 \\
    \method w/o \CGC & 0.904$\pm$0.029 & 0.808$\pm$0.039 & 0.644$\pm$0.078 & \textbf{0.933$\pm$0.041} & 0.747$\pm$0.077 & 0.679$\pm$0.103 \\
    \method w/o \MPP & 0.901$\pm$0.026 & 0.808$\pm$0.035 & 0.648$\pm$0.069 & 0.932$\pm$0.037 & \textbf{0.749$\pm$0.072} & 0.682$\pm$0.096 \\
    \method w/o \MPP \& \CGC & 0.901$\pm$0.026 & 0.807$\pm$0.034 & 0.645$\pm$0.067 & 0.930$\pm$0.045 & 0.749$\pm$0.074 & 0.678$\pm$0.098 \\
    \midrule
    \midrule
    \multirow{2}[4]{*}{} & \multicolumn{3}{c}{\textbf{Ebola}} & \multicolumn{3}{c}{\textbf{Allergy}} \\
    \cmidrule{2-7}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    No Pretrain & 0.967$\pm$0.031 & 0.796$\pm$0.115 & 0.787$\pm$0.113 & 0.994$\pm$0.006 & 0.976$\pm$0.017 & 0.958$\pm$0.019 \\
    \midrule
    ESM-1 & 0.970$\pm$0.035 & 0.845$\pm$0.098 & 0.836$\pm$0.097 & 0.994$\pm$0.006 & 0.988$\pm$0.006 & 0.975$\pm$0.011 \\
    MSA-1b & 0.970$\pm$0.026 & 0.803$\pm$0.103 & 0.799$\pm$0.096 & 0.966$\pm$0.019 & 0.918$\pm$0.037 & 0.835$\pm$0.093 \\
    \midrule
    Ablang-H & 0.951$\pm$0.024 & 0.700$\pm$0.087 & 0.691$\pm$0.079 & 0.821$\pm$0.093 & 0.734$\pm$0.091 & 0.459$\pm$0.190 \\
    Ablang-L & 0.945$\pm$0.027 & 0.719$\pm$0.110 & 0.710$\pm$0.100 & 0.782$\pm$0.136 & 0.735$\pm$0.104 & 0.381$\pm$0.262 \\
    AntiBERT & 0.959$\pm$0.030 & 0.804$\pm$0.110 & 0.795$\pm$0.106 & 0.993$\pm$0.008 & 0.984$\pm$0.009 & 0.970$\pm$0.014 \\
    \midrule
    \method & 0.969$\pm$0.036 & \textbf{0.848$\pm$0.096} & \textbf{0.841$\pm$0.094} & 0.995$\pm$0.006 & \textbf{0.988$\pm$0.005} & \textbf{0.975$\pm$0.011} \\
    \method w/o \CGC & 0.967$\pm$0.032 & 0.843$\pm$0.097 & 0.835$\pm$0.093 & 0.996$\pm$0.004 & 0.983$\pm$0.006 & 0.968$\pm$0.007 \\
    \method w/o \MPP & 0.969$\pm$0.037 & 0.840$\pm$0.094 & 0.828$\pm$0.098 & 0.996$\pm$0.004 & 0.980$\pm$0.005 & 0.961$\pm$0.011 \\
    \method w/o \MPP \& \CGC & \textbf{0.970$\pm$0.025} & 0.821$\pm$0.098 & 0.811$\pm$0.091 & \textbf{0.996$\pm$0.002} & 0.981$\pm$0.007 & 0.963$\pm$0.009 \\
    \midrule
    \midrule
    \multirow{2}[3]{*}{} & \multicolumn{3}{c}{\textbf{SLE}} & \multicolumn{3}{c}{\textbf{MS}} \\
    \cmidrule{2-7}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    No Pretrain & 0.994$\pm$0.004 & 0.982$\pm$0.009 & 0.960$\pm$0.012 & 0.841$\pm$0.182 & 0.847$\pm$0.129 & 0.617$\pm$0.378 \\
    \midrule
    ESM-1 & 0.992$\pm$0.005 & 0.979$\pm$0.014 & 0.954$\pm$0.021 & 0.879$\pm$0.127 & 0.845$\pm$0.123 & 0.621$\pm$0.358 \\
    MSA-1b & \textbf{0.998$\pm$0.001} & \textbf{0.988$\pm$0.007} & \textbf{0.973$\pm$0.011} & 0.853$\pm$0.150 & 0.836$\pm$0.135 & 0.594$\pm$0.392 \\
    \midrule

    Ablang-H & 0.994$\pm$0.003 & 0.964$\pm$0.022 & 0.931$\pm$0.021 & 0.836$\pm$0.184 & 0.828$\pm$0.108 & 0.562$\pm$0.353 \\
    Ablang-L & 0.995$\pm$0.002 & 0.977$\pm$0.017 & 0.956$\pm$0.021 & 0.846$\pm$0.175 & 0.852$\pm$0.115 & 0.633$\pm$0.351 \\
    AntiBERT & 0.994$\pm$0.009 & 0.952$\pm$0.068 & 0.919$\pm$0.096 & \textbf{0.893$\pm$0.095} & \textbf{0.854$\pm$0.112} & \textbf{0.701$\pm$0.214} \\
    \midrule
    \method & 0.990$\pm$0.008 & 0.970$\pm$0.018 & 0.939$\pm$0.018 & 0.847$\pm$0.135 & 0.798$\pm$0.156 & 0.572$\pm$0.294 \\
    \method w/o \CGC & 0.990$\pm$0.007 & 0.962$\pm$0.031 & 0.929$\pm$0.040 & 0.846$\pm$0.132 & 0.799$\pm$0.162 & 0.584$\pm$0.284 \\
    \method w/o \MPP & 0.981$\pm$0.021 & 0.940$\pm$0.063 & 0.891$\pm$0.086 & 0.809$\pm$0.185 & 0.807$\pm$0.152 & 0.535$\pm$0.381 \\
    \method w/o \MPP \& \CGC & 0.988$\pm$0.010 & 0.952$\pm$0.051 & 0.915$\pm$0.070 & 0.827$\pm$0.159 & 0.798$\pm$0.147 & 0.547$\pm$0.311 \\
    \bottomrule
    \end{tabular}%
\end{table}%


==> [arxiv] Antibody/tabs/sequence_level_sars.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease'
\begin{table}[htbp]
  \centering\footnotesize
  \setlength{\tabcolsep}{1.5pt}
  \caption{Sequence-level predictor for SARS-CoV-2.}
  \label{tab:sequence_full}%
    \begin{tabular}{lrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[3]{*}{\textbf{Sequence-level}}} & \multicolumn{3}{c}{\textbf{SARS}}\\
    \cmidrule{2-4}
    & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    No pretrain & 0.894$\pm$0.029 & 0.801$\pm$0.045 & 0.637$\pm$0.078  \\
    ESM-1 & 0.903$\pm$0.061 & 0.799$\pm$0.032 & 0.648$\pm$0.093\\
    MSA-1b & 0.914$\pm$0.025 & 0.810$\pm$0.050 & \textbf{0.671$\pm$0.080}\\
    \midrule
    Ablang-H & 0.915$\pm$0.027 & \textbf{0.817$\pm$0.038} & 0.668$\pm$0.068 \\
    Ablang-L & 0.893$\pm$0.035 & 0.801$\pm$0.054 & 0.637$\pm$0.099 \\
    AntiBERT & \textbf{0.916$\pm$0.026} & 0.810$\pm$0.033 & 0.661$\pm$0.060 \\
    \midrule
    \method & 0.904$\pm$0.027 & 0.808$\pm$0.035 & 0.643$\pm$0.069 \\
    \method w/o \CGC & 0.904$\pm$0.029 & 0.808$\pm$0.039 & 0.644$\pm$0.078 \\
    \method w/o \MPP & 0.901$\pm$0.026 & 0.808$\pm$0.035 & 0.648$\pm$0.069 \\
    \method w/o \MPP \& \CGC & 0.901$\pm$0.026 & 0.807$\pm$0.034 & 0.645$\pm$0.067\\
    \bottomrule
    \end{tabular}%
\end{table}%


==> [arxiv] Antibody/tabs/tasks.tex <==
% Table generated by Excel2LaTeX from sheet 'Dataset'
\begin{table}[htb]
  \centering\footnotesize
  \setlength{\tabcolsep}{3pt}
    \caption{\benchmark benchmark. The five downstream tasks are divided into three biological categories and each category focuses on different input levels. `Q6' indicates the classification task have 6 classes. For disease diagnosis, the size indicate the number of profiles, where each profile contains thousands to millions of sequences.}
    \begin{tabular}{cccccc}
    \toprule
    \textbf{Specificity} & \textbf{Task Name} & \textbf{Input} & \textbf{Formalization} & \textbf{Size} \\
    \midrule
    % \multirow{2}[0]{*}{Therapeutic Antibody Engineering} & Antigen Binding Prediction & CDR fragment & Q2 classification & 35,117  \\
    %   & Paratope Prediction & CDR residue & Q2 labeling & 1,662  \\
    Low & Antigen Binding Prediction & CDR fragment & Q2 Cls. & 21,612 seqs \\
    % \midrule
    Medium  & Paratope Prediction & CDR residue & Q2 Labeling & 1,662 seqs, 21,342 positions \\
    %Disease Diagnosis & Disease Classification & Individual Profile & Q7 classification &  313  \\
    % \midrule
    High  & SARS Antibody Classification & Sequence & Q2 Cls. & 22,000 seqs\\
    High  & B Cell Classification & Sequence & Q6 Cls. & 88,094 seqs \\



%    \multirow{3}[0]{*}{Disease Diagnosis} & SARS/HIV/Ebola & Individual Profile & Q2 classification & 133/51/14  \\
%      & Allergy/SLE/MS  & Individual Profile & Q2 classification & 12/8/8  \\
%      & Disease Classification & Individual Profile & Q7 classification &  313   \\

    \bottomrule
    \end{tabular}%
  \label{tab:task}%
\end{table}%


==> sections/checklist.tex <==

%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}

==> tabs/Pretrained_2.tex <==
% % Table generated by Excel2LaTeX from sheet 'Pretrained'
% \begin{table}[htbp]
%   \centering
%   \caption{Pretrained Model}
%     \begin{tabular}{lrr}
%     \toprule
%     \textbf{Model} & \multicolumn{1}{c}{\textbf{Loss}} & \multicolumn{1}{c}{\textbf{Step}} \\
%     \midrule
%     % BERT & 0.437 & 568000 \\
%     % BERT + contrastive & 0.558 & 19000 \\
%     % BERT + mutation & 1.744 & 134000 \\
%     EALM w/o \MPP \& \CGC  & 0.143 & 108000 \\
%     EALM w/o \CGC & 1.744 & 134000 \\
%     EALM w/o \MPP & 0.001 & 18000 \\    
%     EALM  & 1.856 & 54000 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:pretrain}%
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Pretrained'
\begin{table}[htbp]\footnotesize
  \centering
  \caption{The pretraining details for different models. The `Germline' is the prediction accuracy of \CGC, and the `Position' and `Mutation' are the accuracy of mutation positions and the mutated residues respectively.}
    \begin{tabular}{lcccccc}
    \toprule
    \multicolumn{1}{c}{\textbf{Model}} & \multicolumn{1}{c}{\textbf{Size}}& \multicolumn{1}{c}{\textbf{Loss}} & \multicolumn{1}{c}{\textbf{Step}} & \textbf{Germline} & \textbf{Position} & \textbf{Mutation} \\
    \midrule
    AntiBERT & 85M & 0.437 & 568000 & / & / & / \\
    AntiBERT w \CGC & 85M& 0.558 & 587000 & 0.330 & / & / \\
    AntiBERT w \MPP & 85M& 1.744 & 622000 & / & 0.965 & 0.410 \\
    %\midrule
    %ESM-1 FT & 85M& 0.2636 & 136000 & / & / & / \\
    %ESM-1b FT & 650M & 0.2704 & 278000 & / & / & / \\
    %\midrule
    \midrule
    \method w/o \CGC \& \MPP & 85M& 0.143 & 108000 & / & / & / \\
    \method w/o \CGC & 85M& 1.744 & 134000 & / & 1.000 & 0.443 \\
    \method w/o \MPP & 85M& 0.001 & 126000 & 1.000 & / & / \\
    \method  & 85M & 1.856 & 252500 & 0.9960 & 1.000 & 0.443 \\
    %\midrule
    %\method-large w/o \CGC \& \MPP & 650M & 0.149 & 193000 & / & / & / \\
    %\method-large w/o \CGC & 650M & 1.753 & 267000 & / & 1.000 & 0.438 \\
    %\method-large w/o \MPP & 650M & 0.001 & 200000 & 1.000 & / & / \\
    %\method-large & 650M & 1.773 & 384000 & 0.996 & 1.000 & 0.431 \\
    \bottomrule
    \end{tabular}%
  \label{tab:pretrain}%
\end{table}%



==> tabs/QM9.tex <==
% Table generated by Excel2LaTeX from sheet 'QM9'
\begin{table}[htbp]
  \centering
  \small
  \setlength{\tabcolsep}{2.8pt}
  \centering
 \tabcolsep 3pt
\caption{MAEs of targets on QM9.}
    \begin{tabular}{lcccccccccccc}
    \toprule
    \textbf{Models} & $\mu(D)$ & $\alpha$($a^3_0$) 
    & $\varepsilon_\text{HOMO} $   &  $\varepsilon_\text{LUMO} $ 
    & $\Delta\varepsilon $ & $\langle R^2 \rangle (a_0^3)$ &
    ZPVE   & \textit{$U_0$}  &
    \textit{U} & \textit{H}  &
    \textit{G}   & $C_v(\frac{\text{cal}}{\text{molK}})$ \\ 
    \midrule
    \multirow{1}[0]{*}{MXMNet} & 0.0396 & 0.0447 & 24.7 & 19.7 & 32.6 & 0.512 & 1.15 & 5.90 & 5.94 & 6.09 & 7.17 & 0.0224  \\
    \bottomrule
    \end{tabular}%
  \label{tab:QM9}%
\end{table}%


% Table generated by Excel2LaTeX from sheet 



==> tabs/case_study.tex <==
\begin{table}[b]\footnotesize
 \begin{minipage}[t]{0.55\linewidth}
 \vspace{10pt} % for top [t] alignment, bottom is [b]
    \centering
        \includegraphics[width=\linewidth]{figs/SARS_90.pdf}
        \caption{t90.}
        \label{fig:SARS_90}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.5\linewidth}
      \vspace{0pt}
            \centering
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\textwidth]{figs/health.germtype.pdf}
                \caption{Health germlines.}
                \label{fig:germ_health}
            \end{subfigure}
            % \hfill
            % \hspace{-7mm}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\textwidth]{figs/sars.germtype.pdf}
                \caption{Patient germlines.}
                \label{fig:germ_sars}
            \end{subfigure}
            % \vskip 0.1\baselineskip
            % \hspace{-4mm}
            \begin{subfigure}{0.45\textwidth}
                \includegraphics[width=\textwidth]{figs/health.freq1000.pdf}
                \caption{Health distance.}
                % \vspace{-0.5\baselineskip}
                \label{fig:health_dist}
            \end{subfigure}
            % \hfill
            % \hspace{-8mm}
            \begin{subfigure}{0.45\textwidth}
               \includegraphics[width=\textwidth]{figs/sars.freq1000.pdf}
                \caption{Patient distance.}
                % \vspace{-0.5\baselineskip}
                \label{fig:sars_dist}
            \end{subfigure}
            \caption{UMAP Visualization. (a-b) for sequences with different germlines. One color indicates one germline with its descendant. (c-d) for evolutionary phylogeny distance. The shade of color indicate its distance from the ancestor germline.}
            \label{fig:germline}
  \end{minipage}
\end{table}

==> tabs/cell.tex <==
% Table generated by Excel2LaTeX from sheet 'Cell'
\begin{table}[htbp]
  \centering
  \caption{Cell}
    \begin{tabular}{lr} 
    \toprule
    \textbf{Model} & \multicolumn{1}{c}{\textbf{ACC}} \\
    \midrule
    Ablang-H~\citep{olsen2022ablang} & 0.5695 \\
    Ablang-L~\citep{olsen2022ablang} & 0.5462 \\
    ESM-1b~\citep{rives2021biological} & 0.5030 \\
    \midrule
    Transformer & 0.5542 \\
    AntiBERT & 0.4646 \\
    \midrule
    \method & \textbf{0.5814} \\
    \method w/o \CGC & 0.5593 \\
    \method w/o \MPP & 0.5634 \\
    \method w/o \CGC \& \MPP & 0.5591 \\
    \bottomrule
    \end{tabular}%
  \label{tab:cell}%
\end{table}%


==> tabs/cell_analysis.tex <==
% Table generated by Excel2LaTeX from sheet 'Cell'
% \begin{table}[htbp]
%   \centering\small
%   \setlength{\tabcolsep}{1pt}
%   \caption{Cell Analysis}
%     \begin{tabular}{lcccccc}
%     \toprule
%       & \multicolumn{1}{l}{\textbf{Immature B}} & \multicolumn{1}{l}{\textbf{Memory IgD-}} & \multicolumn{1}{l}{\textbf{Memory IgD+}} & \multicolumn{1}{l}{\textbf{Plasmacytes PC}} & \multicolumn{1}{l}{\textbf{Transitional B}} & \multicolumn{1}{l}{\textbf{Mature B}} \\
%     \midrule
%     \textbf{Immature B} & 89.59 & 1.63 & 1.50 & 1.63 & 4.15 & 1.50 \\
%     \textbf{Memory IgD-} & 2.63 & 50.18 & 9.58 & 15.93 & 7.90 & 13.77 \\
%     \textbf{Memory IgD+} & 1.83 & 5.12 & 44.62 & 17.34 & 12.22 & 18.87 \\
%     \textbf{Plasmacytes PC} & 1.81 & 4.95 & 12.57 & 59.85 & 8.26 & 12.57 \\
%     \textbf{Transitional B} & 3.70 & 4.85 & 16.02 & 18.03 & 40.60 & 16.80 \\
%     \textbf{Mature B} & 2.14 & 5.26 & 15.59 & 18.22 & 13.33 & 45.48 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:cell_analysis}%
% \end{table}%


\begin{table}[b]\footnotesize
 \begin{minipage}[t]{0.45\linewidth}
 \vspace{0pt} % for top [t] alignment, bottom is [b]
    \centering
    \caption{B cell classification (Q6). \textbf{ACC} is the prediction accuracy. The details are in Section \ref{sec:task} and \ref{sec:method}. The best result is bolded.}
   \label{tab:cell}%
   \footnotesize\setlength{\tabcolsep}{3pt}
    \begin{tabular}{lr}
        \toprule
        \textbf{Model} & \multicolumn{1}{c}{\textbf{ACC}} \\
        \midrule
        No Pretrain & 0.554 $\pm$ 0.042\\
        \midrule
        ESM-1~\citep{rives2021biological} & 0.503 $\pm$ 0.031 \\
        ESM-1 FT \\
        MSA-1b~\citep{rao2021msa} & 0.416 $\pm$ 0.050 \\
        \midrule
        Ablang-H~\citep{olsen2022ablang} & 0.570 $\pm$ 0.010 \\
        Ablang-L~\citep{olsen2022ablang} & 0.546 $\pm$ 0.008 \\
        AntiBERT & 0.565 $\pm$ 0.028\\
        \midrule
        %Transformer & 0.554 $\pm$ 0.042\\
        \method & \textbf{0.581 $\pm$ 0.005} \\
        \method w/o \CGC & 0.559 $\pm$ 0.012 \\
        \method w/o \MPP & 0.563 $\pm$ 0.010 \\
        \method w/o \CGC \& \MPP & 0.559 $\pm$ 0.009\\
        \bottomrule
    \end{tabular}%
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.5\linewidth}
  \vspace{0pt}
      \centering
    %   \begin{figure}
        \includegraphics[width=\textwidth]{figs/cell.pdf}
        \caption{Category prediction. For each $p_{ij}$ in $i-$th row and $j$-th column, it means the frequency for the model to predict a sequence in $i$ category to $j$ category. The number is normalized by row.}
        \label{fig:cell_analysis}
    % \end{figure}
  \end{minipage}
\end{table}


==> tabs/disease.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease'
\begin{table}[t]
  \centering\footnotesize
  \setlength{\tabcolsep}{2pt}
  \caption{Disease Diagnosis. The definition of notation \textbf{AUC}, \textbf{F1}, \textbf{MCC} can be found in Section \ref{sec:benchmark}. The full table with more diseases and standard deviations can be found in Appendix.}
  
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[1]{*}{\textbf{Individual-level}}} & \multicolumn{3}{c}{\textbf{SARS}} & \multicolumn{3}{c}{\textbf{HIV}} & \multicolumn{3}{c}{\textbf{Ebola}} \\
    \cmidrule{2-10}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    Ablang-H & 0.988 & 0.968 & 0.920 & 0.960 & 0.788 & 0.744 & 0.944 & 0.767 & 0.750 \\
    Ablang-L & \textbf{0.990} & 0.938 & 0.843 & 0.931 & 0.798 & 0.742 & 0.961 & 0.731 & 0.703 \\
    ESM-1 & 0.979 & 0.933 & 0.824 & 0.967 & 0.883 & 0.849 & \textbf{1.000} & 0.933 & 0.934 \\
    MSA-1b & 0.989 & 0.954 & 0.887 & 0.962 & 0.833 & 0.789 & \textbf{1.000} & 0.933 & 0.934 \\
    \midrule
    Transformer & 0.975 & 0.962 & 0.902 & 0.920 & 0.815 & 0.776 & 0.994 & 0.933 & 0.934 \\
    AntiBERT & 0.983 & 0.976 & 0.938 & 0.969 & 0.878 & 0.850 & 0.978 & 0.933 & 0.934 \\
    \midrule
    \method & 0.977 & \textbf{0.983} & \textbf{0.955} & \textbf{0.978} & 0.914 & 0.884 & \textbf{1.000} & \textbf{0.947} & \textbf{0.944} \\
    \method w/o \CGC & 0.983 & 0.973 & 0.929 & \textbf{0.978} & 0.903 & 0.869 & \textbf{1.000} & 0.933 & 0.934 \\
    \method w/o \MPP & 0.987 & 0.969 & 0.921 & 0.976 & 0.906 & 0.880 & \textbf{1.000} & 0.933 & 0.934 \\
    \method w/o \CGC \& \MPP & 0.986 & 0.969 & 0.920 & 0.973 & \textbf{0.919} & \textbf{0.896} & 0.994 & 0.933 & 0.934 \\
    \bottomrule
    \end{tabular}%
  \label{tab:disease}%
\end{table}%


==> tabs/disease_seq.tex <==
% Table generated by Excel2LaTeX from sheet 'Disease'
\begin{table}[htbp]
  \centering\footnotesize
  \setlength{\tabcolsep}{3pt}
  \caption{Sequence-level predictor for disease diagnosis. The definition of notation are the same as the Table 4 in main body.}
    \begin{tabular}{lrrrrrrrrr}
    \toprule
    \multicolumn{1}{c}{\multirow{2}[1]{*}{\textbf{Sequence-level}}} & \multicolumn{3}{c}{\textbf{SARS}} & \multicolumn{3}{c}{\textbf{HIV}} & \multicolumn{3}{c}{\textbf{Ebola}} \\
    \cmidrule{2-10}  & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} & \multicolumn{1}{c}{\textbf{AUC}} & \multicolumn{1}{c}{\textbf{F1}} & \multicolumn{1}{c}{\textbf{MCC}} \\
    \midrule
    Ablang-H & 0.9151 & \textbf{0.8166} & \textbf{0.6679} & 0.8948 & 0.6842 & 0.6036 & 0.9514 & 0.7003 & 0.6908 \\
    Ablang-L & 0.8929 & 0.8012 & 0.6372 & 0.8813 & 0.6682 & 0.5842 & 0.9450 & 0.7185 & 0.7096 \\
    ESM-1b & 0.9032 & 0.7992 & 0.6476 & 0.9268 & 0.7386 & \textbf{0.7008} & \textbf{0.9704} & 0.8447 & 0.8357 \\
    \midrule
    Transformer & 0.8939 & 0.8007 & 0.6367 & 0.8928 & 0.6224 & 0.5625 & 0.9665 & 0.7960 & 0.7869 \\
    AntiBERT & \textbf{0.9155} & 0.8101 & 0.6606 & 0.9213 & 0.7422 & 0.6893 & 0.9591 & 0.8043 & 0.7952 \\
    \midrule
    \method & 0.9043 & 0.8081 & 0.6434 & 0.9297 & 0.7438 & 0.6768 & 0.9689 & \textbf{0.8484} & \textbf{0.8407} \\
    \method w/o \CGC & 0.9040 & 0.8083 & 0.6442 & \textbf{0.9326} & 0.7473 & 0.6786 & 0.9671 & 0.8426 & 0.8346 \\
    \method w/o \MPP & 0.9011 & 0.8081 & 0.6484 & 0.9319 & 0.7485 & 0.6822 & 0.9694 & 0.8404 & 0.8284 \\
    \method w/o \CGC \& \MPP & 0.9010 & 0.8074 & 0.6446 & 0.9303 & \textbf{0.7492} & 0.6784 & 0.9699 & 0.8208 & 0.8113 \\
    \bottomrule
    \end{tabular}%
  \label{tab:disease_seq}%
\end{table}%




==> tabs/newbinder.tex <==
% Table generated by Excel2LaTeX from sheet 'New binder'

\begin{table}[htbp]\footnotesize
   \setlength{\tabcolsep}{2.8pt}
  \centering
  \caption{The CDR3-H3 region of high-ranked sequences to bind to SARS. We show the CDR3 fragment of the heavy chain in the antibody sequences. `Identity' is the similarity between the predicted binder and the true binder. The epitope of the true binders are shown. The difference amino acids between predicted binder and true binder are highlighted in red}
  %Binder No.16 comes from semi-synthetic library and binind No. 32 and No. 34 from Phage display. 'unk' stands for unknown.}
    \begin{tabular}{rlllcc}
    \toprule
    \textbf{No}  & \textbf{Predicted Binder} & \textbf{Existing Binder} & \textbf{Epitope} & \textbf{Identity $\uparrow$ } \\
    \midrule
    1 & AREGIVGATTGFDY & AREGIVGATTGFDY & spike & 1.000 \\
    2 & ARDLGGYFDY & ARDLGGYFDY & RBD & 1.000 \\
    3 & AKDQDD\textcolor{red}{A}YYYYYYMDV & AKDQDD\textcolor{red}{G}YYYYYYMDV & NTD & 0.938 \\
    4 & ASYYYDSSGY\textcolor{red}{H}YGMDV & ASYYYDSSGY\textcolor{red}{Y}YGMDV & RBD & 0.938 \\
    5 & ARRG\textcolor{red}{L}GLYYYGMDV & ARRG\textcolor{red}{D}GLYYYGMDV & S2 & 0.929 \\
    6 & ARA\textcolor{red}{F}RGSYYYGMDV & ARA\textcolor{red}{T}RGSYYYGMDV & S2 & 0.929 \\
    7 & ARLSGSSW\textcolor{red}{Y}FDY & ARLSGSSW\textcolor{red}{D}FDY & spike & 0.917 \\
    8 & AR\textcolor{red}{L}GSSSWYFDY & AR\textcolor{red}{V}GSSSWYFDY & spike & 0.917 \\
    9 & AR\textcolor{red}{-}GWLRGYFDL & AR\textcolor{red}{R}GWLRGYFDL & RBD & 0.909 \\
    10 & ARDWGE\textcolor{red}{L}YFDY & ARDWGE\textcolor{red}{Y}YFDY & RBD & 0.909 \\
    11 & ARDLGG\textcolor{red}{V}FDY & ARDLGG\textcolor{red}{Y}FDY & RBD & 0.900 \\
    %12 & ARGDSSGWYTGDVFDI & ARVDSSGWYTGDVFDV & RBD & 0.875 \\
    %13 & ARGDSDSSGYYYYFDY & ARGDSSGYYYYFDY & RBD & 0.871 \\
    %14 & ARHRAAGGNYYYGMDV & ARAAGGNYYYGMDV & RBD & 0.875 \\
    %15 & AAPYCSGGSCTDAFDI & AAPYCSGGSCFDAFDM & RBD & 0.875 \\
    %16 & AKDRYYYDSSGYYEYYYYYGMDV & ARDRYYYDSSGYYYDYYYGMDV & RBD & 0.870 \\
    %17 & AKGDTAMAPYNWFDP & AKADTAMAWYNWFDP & NTD & 0.867 \\
    %18 & ARAPGSSYSSGWYDYYYGMDV & ARAPGASYSSGWYHYYYYMDV & RBD & 0.857 \\
    %19 & ATGVAVAGTPRYYYYYYGMDV & ATGVAVAGTPSSYYYYYYMDV & spike & 0.857 \\
    %20 & AVNSNYYYYYGMDV & ARYSNYYYYYGMDV & NTD & 0.857 \\
    %21 & ASYQNYYYYYGMDV & ARYSNYYYYYGMDV & NTD & 0.857 \\
    %22 & ARPRSGSYRDYFDY & ARPRSGSYYAYFDY & spike & 0.857 \\
    %23 & ARARGGSYLYGMDV & ARARGGNYYYGMDV & S2 & 0.857 \\
    %24 & ARSYSGSYYSRFDY & ARTYSGSYYSYFDY & S2 & 0.857 \\
    %25 & ARPFGGSYYSGFDY & ARPHGGSYYSYFDY & S2 & 0.857 \\
    %26 & ASGIAATYYYYMDV & ARGPAATYYYYMDV & spike & 0.857 \\
    %27 & AKDRAGNYYYGMDV & ARDRSGNYYYGMDV & spike & 0.857 \\
    %28 & ARDGIVGATTGLDY & ARDGMVGATTGIDY & S2 & 0.857 \\
    %29 & ARNRGGSYLGAFDI & ARARGGSYSGAFDI & unk & 0.857 \\
    %30 & ARGNSSGWSYYFDY & ARGDSNGWSYYFDY & spike & 0.857 \\
    %31 & ARLGSGSYSNWFDP & ARSGSGSYFNWFDP & S2 & 0.857 \\
    %32 & ARAMGGSYYGGMDV & ARARGGSYYYGMDV & S2 & 0.857 \\
    %33 & ARPTSGGYYYGMDV & ARAYSGGYYYGMDV & S2 & 0.857 \\
    %34 & ATSAVAGTPNWFDP & ATSRVAGTPNWFHP & NTD & 0.857 \\
    %35 & AREDYYDSSGAFDI & AREDYYDSSGSFDH & RBD & 0.857 \\
    %36 & ARRGHGLYYHGMDV & ARRGDGLYYYGMDV & unk & 0.857 \\
    %37 & ARDRGYCSSTSCYYYYGMDV & ARDDIGYCSSTSCSYYYYGMDV & spike & 0.850 \\
    \bottomrule
    \end{tabular}%
  \label{tab:newbinder}%
\end{table}%





==> tabs/newbinder2.tex <==
% Table generated by Excel2LaTeX from sheet 'sars.highprob08.sorted.uniq'
\begin{table}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{rllrr}
      \textbf{No}  & \textbf{CDR-H3 of predicted binder} & \textbf{CDR-H3 of  true binder} & \textbf{Identity} & \textbf{Score} \\
    1 & AREGIVGATTGFDY & AREGIVGATTGFDY & 1.0000 & 1.0000 \\
    2 & ARDLGGYFDY & ARDLGGYFDY & 1.0000 & 1.0000 \\
    3 & ARDLGGYFDY &  ARDLGGYFDY & 0.9312 & 1.0000 \\
    4 & AKDQDDAYYYYYYMDV & AKDQDDGYYYYYYMDV & 0.9645 & 0.9375 \\
    5 & ASYYYDSSGYHYGMDV & ASYYYDSSGYYYGMDV & 0.8858 & 0.9375 \\
    6 & ARRGLGLYYYGMDV & ARRGDGLYYYGMDV & 1.0000 & 0.9286 \\
    7 & ARAFRGSYYYGMDV & ARATRGSYYYGMDV & 1.0000 & 0.9286 \\
    8 & ARLSGSSWYFDY & ARLSGSSWDFDY & 0.9765 & 0.9167 \\
    9 & ARLGSSSWYFDY & ARVGSSSWYFDY & 0.9344 & 0.9167 \\
    10 & ARGWLRGYFDL & ARRGWLRGYFDL & 0.9996 & 0.9091 \\
    11 & ARDWGELYFDY & ARDWGEYYFDY & 0.8164 & 0.9091 \\
    12 & ARGDSSGWYTGDVFDI & ARVDSSGWYTGDVFDV & 1.0000 & 0.8750 \\
    13 & ARGDSDSSGYYYYFDY & ARGDSSGYYYYFDY & 1.0000 & 0.8750 \\
    14 & ARHRAAGGNYYYGMDV & ARAAGGNYYYGMDV & 0.9218 & 0.8750 \\
    15 & AAPYCSGGSCTDAFDI & AAPYCSGGSCFDAFDM & 0.8742 & 0.8750 \\
    16 & AKDRYYYDSSGYYEYYYYYGMDV & ARDRYYYDSSGYYYDYYYGMDV & 0.9968 & 0.8696 \\
    17 & AKGDTAMAPYNWFDP & AKADTAMAWYNWFDP & 1.0000 & 0.8667 \\
    18 & ARAPGSSYSSGWYDYYYGMDV & ARAPGASYSSGWYHYYYYMDV & 1.0000 & 0.8571 \\
    19 & ATGVAVAGTPRYYYYYYGMDV & ATGVAVAGTPSSYYYYYYMDV & 1.0000 & 0.8571 \\
    20 & AVNSNYYYYYGMDV & ARYSNYYYYYGMDV & 0.9999 & 0.8571 \\
    21 & ASYQNYYYYYGMDV & ARYSNYYYYYGMDV & 0.9981 & 0.8571 \\
    22 & ARPRSGSYRDYFDY & ARPRSGSYYAYFDY & 0.9925 & 0.8571 \\
    23 & ARARGGSYLYGMDV & ARARGGNYYYGMDV & 0.9922 & 0.8571 \\
    24 & ARSYSGSYYSRFDY & ARTYSGSYYSYFDY & 0.9819 & 0.8571 \\
    25 & ARPFGGSYYSGFDY & ARPHGGSYYSYFDY & 0.9738 & 0.8571 \\
    26 & ASGIAATYYYYMDV & ARGPAATYYYYMDV & 0.9677 & 0.8571 \\
    27 & AKDRAGNYYYGMDV & ARDRSGNYYYGMDV & 0.9365 & 0.8571 \\
    28 & ARDGIVGATTGLDY & ARDGMVGATTGIDY & 0.9365 & 0.8571 \\
    29 & ARNRGGSYLGAFDI & ARARGGSYSGAFDI & 0.9101 & 0.8571 \\
    30 & ARGNSSGWSYYFDY & ARGDSNGWSYYFDY & 0.9096 & 0.8571 \\
    31 & ARLGSGSYSNWFDP & ARSGSGSYFNWFDP & 0.8885 & 0.8571 \\
    32 & ARAMGGSYYGGMDV & ARARGGSYYYGMDV & 0.8786 & 0.8571 \\
    33 & ARPTSGGYYYGMDV & ARAYSGGYYYGMDV & 0.8779 & 0.8571 \\
    34 & ARDRGYCSSTSCYYYYGMDV & ARDDIGYCSSTSCSYYYYGMDV & 0.9499 & 0.8500 \\
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%

